Optomechanical disk resonator in the quantum ground state of motion

Although they have enabled several advances in the field of optomechanics, optomechanical disk resonators have not yet been operated in the quantum regime. We present the first experimental demonstration of an optomechanical disk resonator prepared in the quantum ground state. With a gigahertz frequency, the mechanical breathing mode of the investigated semiconductor disk reaches a level of excitation below a single phonon when cooled in a dilution refrigerator. We quantify the phonon occupancy of the mechanical mode by performing Brillouin sideband spectroscopy: a conical optical fiber is evanescently coupled to the disk optical whispering-gallery mode, and Stokes and anti-Stokes photons scattered by phonon emission and absorption are counted on a single-photon detector. We measure a suppression of the absorption process corresponding to a phonon occupancy of $0.66\pm0.20$. We experimentally investigate the mechanisms ruling laser-induced heating, which limits the lowest measurable phonon occupancy, and notably witness an extra-cavity heating effect.

==> biblio.tex <==
@article{aspelmeyer_cavity_2014,
	title = {Cavity optomechanics},
	volume = {86},
	url = {https://link.aps.org/doi/10.1103/RevModPhys.86.1391},
	doi = {10.1103/RevModPhys.86.1391},
	abstract = {The field of cavity optomechanics is reviewed. This field explores the interaction between electromagnetic radiation and nanomechanical or micromechanical motion. This review covers the basics of optical cavities and mechanical resonators, their mutual optomechanical interaction mediated by the radiation-pressure force, the large variety of experimental systems which exhibit this interaction, optical measurements of mechanical motion, dynamical backaction amplification and cooling, nonlinear dynamics, multimode optomechanics, and proposals for future cavity-quantum-optomechanics experiments. In addition, the perspectives for fundamental quantum physics and for possible applications of optomechanical devices are described.},
	number = {4},
	urldate = {2025-04-03},
	journal = {Reviews of Modern Physics},
	author = {Aspelmeyer, Markus and Kippenberg, Tobias J. and Marquardt, Florian},
	month = dec,
	year = {2014},
	pages = {1391--1452},
	file = {APS Snapshot:C\:\\Users\\abarbero\\Zotero\\storage\\BES4DSDT\\RevModPhys.86.html:text/html;Full Text PDF:C\:\\Users\\abarbero\\Zotero\\storage\\8H235JJ6\\Aspelmeyer et al. - 2014 - Cavity optomechanics.pdf:application/pdf},
}

@article{favero_optomechanics_2009,
	title = {Optomechanics of deformable optical cavities},
	volume = {3},
	copyright = {2009 Springer Nature Limited},
	issn = {1749-4893},
	url = {https://www.nature.com/articles/nphoton.2009.42},
	doi = {10.1038/nphoton.2009.42},
	abstract = {Resonant optical cavities such as Fabry–Perot resonators or whispering-gallery structures are subject to radiation pressure pushing their reflecting 'walls' apart. Deformable optical cavities yield to this pressure, but in doing so they in turn affect the stored optical energy, resulting in an optical back-action. For such cavities the optics and the mechanics become strongly coupled, making them fascinating systems in which to explore theories of measurements at the quantum limit. Here we provide a summary of the current state of optomechanics of deformable optical cavities, identifying some of the most important recent developments in the field.},
	language = {en},
	number = {4},
	urldate = {2025-09-25},
	journal = {Nature Photonics},
	author = {Favero, Ivan and Karrai, Khaled},
	month = apr,
	year = {2009},
	pages = {201--205},
}

@article{barzanjeh_optomechanics_2022,
	title = {Optomechanics for quantum technologies},
	volume = {18},
	copyright = {2021 Springer Nature Limited},
	issn = {1745-2481},
	url = {https://www.nature.com/articles/s41567-021-01402-0},
	doi = {10.1038/s41567-021-01402-0},
	abstract = {The ability to control the motion of mechanical systems through interaction with light has opened the door to a plethora of applications in fundamental and applied physics. With experiments routinely reaching the quantum regime, the focus has now turned towards creating and exploiting interesting non-classical states of motion and entanglement in optomechanical systems. Quantumness has also shifted from being the very reason why experiments are constructed to becoming a resource for the investigation of fundamental physics and the creation of quantum technologies. Here, by focusing on opto- and electromechanical platforms we review recent progress in quantum state preparation and entanglement of mechanical systems, together with applications to signal processing and transduction, quantum sensing and topological physics, as well as small-scale thermodynamics.},
	language = {en},
	number = {1},
	urldate = {2025-09-25},
	journal = {Nature Physics},
	author = {Barzanjeh, Shabir and Xuereb, André and Gröblacher, Simon and Paternostro, Mauro and Regal, Cindy A. and Weig, Eva M.},
	month = jan,
	year = {2022},
	pages = {15--24},
	file = {Full Text PDF:C\:\\Users\\abarbero\\Zotero\\storage\\IL2KWQT3\\Barzanjeh et al. - 2022 - Optomechanics for quantum technologies.pdf:application/pdf},
}

@article{degen_quantum_2017,
	title = {Quantum sensing},
	volume = {89},
	url = {https://link.aps.org/doi/10.1103/RevModPhys.89.035002},
	doi = {10.1103/RevModPhys.89.035002},
	abstract = {“Quantum sensing” describes the use of a quantum system, quantum properties, or quantum phenomena to perform a measurement of a physical quantity. Historical examples of quantum sensors include magnetometers based on superconducting quantum interference devices and atomic vapors or atomic clocks. More recently, quantum sensing has become a distinct and rapidly growing branch of research within the area of quantum science and technology, with the most common platforms being spin qubits, trapped ions, and flux qubits. The field is expected to provide new opportunities—especially with regard to high sensitivity and precision—in applied physics and other areas of science. This review provides an introduction to the basic principles, methods, and concepts of quantum sensing from the viewpoint of the interested experimentalist.},
	number = {3},
	urldate = {2025-08-13},
	journal = {Reviews of Modern Physics},
	author = {Degen, C. L. and Reinhard, F. and Cappellaro, P.},
	month = jul,
	year = {2017},
	pages = {035002},
	file = {APS Snapshot:C\:\\Users\\abarbero\\Zotero\\storage\\E9GKKFW6\\RevModPhys.89.html:text/html;Full Text PDF:C\:\\Users\\abarbero\\Zotero\\storage\\RV42KG3P\\Degen et al. - 2017 - Quantum sensing.pdf:application/pdf},
}

@article{pirkkalainen_squeezing_2015,
	title = {Squeezing of {Quantum} {Noise} of {Motion} in a {Micromechanical} {Resonator}},
	volume = {115},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.115.243601},
	doi = {10.1103/PhysRevLett.115.243601},
	abstract = {A pair of conjugate observables, such as the quadrature amplitudes of harmonic motion, have fundamental fluctuations that are bound by the Heisenberg uncertainty relation. However, in a squeezed quantum state, fluctuations of a quantity can be reduced below the standard quantum limit, at the cost of increased fluctuations of the conjugate variable. Here we prepare a nearly macroscopic moving body, realized as a micromechanical resonator, in a squeezed quantum state. We obtain squeezing of one quadrature amplitude 1.1±0.4 dB below the standard quantum limit, thus achieving a long-standing goal of obtaining motional squeezing in a macroscopic object.},
	number = {24},
	urldate = {2025-09-25},
	journal = {Physical Review Letters},
	author = {Pirkkalainen, J.-M. and Damskägg, E. and Brandt, M. and Massel, F. and Sillanpää, M. A.},
	month = dec,
	year = {2015},
	pages = {243601},
	file = {APS Snapshot:C\:\\Users\\abarbero\\Zotero\\storage\\CCWI4S27\\PhysRevLett.115.html:text/html;Full Text PDF:C\:\\Users\\abarbero\\Zotero\\storage\\TMDZE7XE\\Pirkkalainen et al. - 2015 - Squeezing of Quantum Noise of Motion in a Micromechanical Resonator.pdf:application/pdf},
}

@article{marti_quantum_2024,
	title = {Quantum squeezing in a nonlinear mechanical oscillator},
	volume = {20},
	copyright = {2024 The Author(s)},
	issn = {1745-2481},
	url = {https://www.nature.com/articles/s41567-024-02545-6},
	doi = {10.1038/s41567-024-02545-6},
	abstract = {Mechanical degrees of freedom are natural candidates for continuous-variable quantum information processing and bosonic quantum simulations. However, these applications require the engineering of squeezing and nonlinearities in the quantum regime. Here we demonstrate squeezing below the zero-point fluctuations of a gigahertz-frequency mechanical resonator coupled to a superconducting qubit. This is achieved by parametrically driving the qubit, which results in an effective two-phonon drive. In addition, we show that the resonator mode inherits a nonlinearity from the off-resonant coupling with the qubit, which can be tuned by controlling the detuning. We, thus, realize a mechanical squeezed Kerr oscillator, in which we demonstrate the preparation of non-Gaussian quantum states of motion with Wigner function negativities and high quantum Fisher information. This shows that our results can also have applications in quantum metrology and sensing.},
	language = {en},
	number = {9},
	urldate = {2025-08-13},
	journal = {Nature Physics},
	author = {Marti, Stefano and von Lüpke, Uwe and Joshi, Om and Yang, Yu and Bild, Marius and Omahen, Andraz and Chu, Yiwen and Fadel, Matteo},
	month = sep,
	year = {2024},
	pages = {1448--1453},
	file = {Full Text PDF:C\:\\Users\\abarbero\\Zotero\\storage\\XRK8B4SC\\Marti et al. - 2024 - Quantum squeezing in a nonlinear mechanical oscillator.pdf:application/pdf},
}

@article{pan_realization_2025,
	title = {Realization of {Versatile} and {Effective} {Quantum} {Metrology} {Using} a {Single} {Bosonic} {Mode}},
	volume = {6},
	url = {https://link.aps.org/doi/10.1103/PRXQuantum.6.010304},
	doi = {10.1103/PRXQuantum.6.010304},
	abstract = {Quantum metrology offers the potential to surpass its classical counterpart, pushing the boundaries of measurement precision toward the ultimate Heisenberg limit. This enhanced precision is normally attained by utilizing large squeezed states or multiparticle entangled quantum states, both of which are often challenging to implement and prone to decoherence in real quantum devices. In this work, we present a versatile and on-demand protocol for deterministic parameter estimation that leverages two efficient state-transfer operations on a single bosonic mode. Specifically, we demonstrate this protocol in the context of phase estimation using the superposition of coherent states in the bosonic circuit quantum electrodynamics (cQED) platform. With low average photon numbers of only up to 1.76, we achieve quantum enhanced precision approaching the Heisenberg scaling, reaching a metrological gain of 7.5⁢(6) dB. Importantly, we show that the gain or sensitivity range can be further enhanced on the fly by tailoring the input states, with different superposition weights, based on specific system constraints. The realization of this versatile and efficient scheme affords a promising path toward practical quantum enhanced sensing, not only for bosonic cQED hardware but also readily extensible to other continuous-variable platforms.},
	number = {1},
	urldate = {2025-09-25},
	journal = {PRX Quantum},
	author = {Pan, Xiaozhou and Krisnanda, Tanjung and Duina, Andrea and Park, Kimin and Song, Pengtao and Fontaine, Clara Yun and Copetudo, Adrian and Filip, Radim and Gao, Yvonne Y.},
	month = jan,
	year = {2025},
	pages = {010304},
	file = {APS Snapshot:C\:\\Users\\abarbero\\Zotero\\storage\\57W8J869\\PRXQuantum.6.html:text/html;Full Text PDF:C\:\\Users\\abarbero\\Zotero\\storage\\UPQ65NTB\\Pan et al. - 2025 - Realization of Versatile and Effective Quantum Metrology Using a Single Bosonic Mode.pdf:application/pdf},
}

@article{julsgaard_experimental_2004,
	title = {Experimental demonstration of quantum memory for light},
	volume = {432},
	copyright = {2004 Macmillan Magazines Ltd.},
	issn = {1476-4687},
	url = {https://www.nature.com/articles/nature03064},
	doi = {10.1038/nature03064},
	abstract = {The information carrier of today's communications, a weak pulse of light, is an intrinsically quantum object. As a consequence, complete information about the pulse cannot be perfectly recorded in a classical memory, even in principle. In the field of quantum information, this has led to the long-standing challenge of how to achieve a high-fidelity transfer of an independently prepared quantum state of light onto an atomic quantum state1,2,3,4. Here we propose and experimentally demonstrate a protocol for such a quantum memory based on atomic ensembles. Recording of an externally provided quantum state of light onto the atomic quantum memory is achieved with 70 per cent fidelity, significantly higher than the limit for classical recording. Quantum storage of light is achieved in three steps: first, interaction of the input pulse and an entangling field with spin-polarized caesium atoms; second, subsequent measurement of the transmitted light; and third, feedback onto the atoms using a radio-frequency magnetic pulse conditioned on the measurement result. The density of recorded states is 33 per cent higher than the best classical recording of light onto atoms, with a quantum memory lifetime of up to 4 milliseconds.},
	language = {en},
	number = {7016},
	urldate = {2025-08-13},
	journal = {Nature},
	author = {Julsgaard, Brian and Sherson, Jacob and Cirac, J. Ignacio and Fiurášek, Jaromír and Polzik, Eugene S.},
	month = nov,
	year = {2004},
	pages = {482--486},
	file = {Full Text PDF:C\:\\Users\\abarbero\\Zotero\\storage\\Q7SSHC73\\Julsgaard et al. - 2004 - Experimental demonstration of quantum memory for light.pdf:application/pdf},
}

@article{deplano_high_2025,
	title = {High purity two-dimensional levitated mechanical oscillator},
	volume = {16},
	copyright = {2025 The Author(s)},
	issn = {2041-1723},
	url = {https://www.nature.com/articles/s41467-025-59213-3},
	doi = {10.1038/s41467-025-59213-3},
	abstract = {In recent years, levitated optomechanics has delivered on the promise of reaching the motional quantum ground state. An important next milestone of the field would be the generation of mechanical entanglement. An ideal candidate is the two-dimensional motion in the polarization plane of an optical tweezer inside an optical cavity, where optical and mechanical modes are coupled via coherent scattering. Achieving this goal requires two key conditions: two-dimensional ground state cooling along with substantial spectral overlap between the two modes. The latter is essential to generate the necessary correlations, but unfortunately, it hinders efficient cooling thus narrowing the useful parameter space. In this work, we report the achievement of a high purity two-dimensional state in a regime where the strong optomechanical coupling induces the desired spectral overlap between oscillations in different directions, as reflected in the non-trivial spectral shape of the detected cavity field. As a result, significant correlations consistently arise between any pair of orthogonal directions, preventing the motion from being reduced to two independent one-dimensional oscillators and leading to higher purity compared to that scenario. Our system serves as an excellent platform for realizing continuous variable entanglement in two-dimensional motion.},
	language = {en},
	number = {1},
	urldate = {2025-09-25},
	journal = {Nature Communications},
	author = {Deplano, Q. and Pontin, A. and Ranfagni, A. and Marino, F. and Marin, F.},
	month = may,
	year = {2025},
	pages = {4215},
	file = {Full Text PDF:C\:\\Users\\abarbero\\Zotero\\storage\\FKHLTZ4H\\Deplano et al. - 2025 - High purity two-dimensional levitated mechanical oscillator.pdf:application/pdf},
}

@article{seis_ground_2022,
	title = {Ground state cooling of an ultracoherent electromechanical system},
	volume = {13},
	copyright = {2022 The Author(s)},
	issn = {2041-1723},
	url = {https://www.nature.com/articles/s41467-022-29115-9},
	doi = {10.1038/s41467-022-29115-9},
	abstract = {Cavity electromechanics relies on parametric coupling between microwave and mechanical modes to manipulate the mechanical quantum state, and provide a coherent interface between different parts of hybrid quantum systems. High coherence of the mechanical mode is of key importance in such applications, in order to protect the quantum states it hosts from thermal decoherence. Here, we introduce an electromechanical system based around a soft-clamped mechanical resonator with an extremely high Q-factor ({\textgreater}109) held at very low (30 mK) temperatures. This ultracoherent mechanical resonator is capacitively coupled to a microwave mode, strong enough to enable ground-state-cooling of the mechanics (\$\$\{{\textbackslash}bar\{n\}\}\_\{{\textbackslash}min \}=0.76{\textbackslash}pm 0.16\$\$). This paves the way towards exploiting the extremely long coherence times (tcoh {\textgreater} 100 ms) offered by such systems for quantum information processing and state conversion.},
	language = {en},
	number = {1},
	urldate = {2025-09-25},
	journal = {Nature Communications},
	author = {Seis, Yannick and Capelle, Thibault and Langman, Eric and Saarinen, Sampo and Planz, Eric and Schliesser, Albert},
	month = mar,
	year = {2022},
	pages = {1507},
	file = {Full Text PDF:C\:\\Users\\abarbero\\Zotero\\storage\\7FFC26V8\\Seis et al. - 2022 - Ground state cooling of an ultracoherent electromechanical system.pdf:application/pdf},
}

@article{riedinger_non-classical_2016,
	title = {Non-classical correlations between single photons and phonons from a mechanical oscillator},
	volume = {530},
	copyright = {2016 Springer Nature Limited},
	issn = {1476-4687},
	url = {https://www.nature.com/articles/nature16536},
	doi = {10.1038/nature16536},
	abstract = {Non-classically correlated pairs of single photons and phonons are generated and read out from a nanomechanical resonator, demonstrating that such resonators could be used for light–matter quantum interfaces.},
	language = {en},
	number = {7590},
	urldate = {2025-08-13},
	journal = {Nature},
	author = {Riedinger, Ralf and Hong, Sungkun and Norte, Richard A. and Slater, Joshua A. and Shang, Juying and Krause, Alexander G. and Anant, Vikas and Aspelmeyer, Markus and Gröblacher, Simon},
	month = feb,
	year = {2016},
	pages = {313--316},
	file = {Full Text PDF:C\:\\Users\\abarbero\\Zotero\\storage\\MP99LSTG\\Riedinger et al. - 2016 - Non-classical correlations between single photons and phonons from a mechanical oscillator.pdf:application/pdf},
}

@article{chu_creation_2018,
	title = {Creation and control of multi-phonon {Fock} states in a bulk acoustic-wave resonator},
	volume = {563},
	copyright = {2018 Springer Nature Limited},
	issn = {1476-4687},
	url = {https://www.nature.com/articles/s41586-018-0717-7},
	doi = {10.1038/s41586-018-0717-7},
	abstract = {Quantum states of mechanical motion can be important resources for quantum information, metrology and studies of fundamental physics. Recent demonstrations of superconducting qubits coupled to acoustic resonators have opened up the possibility of performing quantum operations on macroscale motional modes1–3, which can act as long-lived quantum memories or transducers. In addition, they can potentially be used to test decoherence mechanisms in macroscale objects and other modifications to standard quantum theory4,5. Many of these applications call for the ability to create and characterize complex quantum states, such as states with a well defined phonon number, also known as phonon Fock states. Such capabilities require fast quantum operations and long coherence times of the mechanical mode. Here we demonstrate the controlled generation of multi-phonon Fock states in a macroscale bulk acoustic-wave resonator. We also perform Wigner tomography and state reconstruction to highlight the quantum nature of the prepared states6. These demonstrations are made possible by the long coherence times of our acoustic resonator and our ability to selectively couple a superconducting qubit to individual phonon modes. Our work shows that circuit quantum acoustodynamics7 enables sophisticated quantum control of macroscale mechanical objects and opens up the possibility of using acoustic modes as quantum resources.},
	language = {en},
	number = {7733},
	urldate = {2025-08-13},
	journal = {Nature},
	author = {Chu, Yiwen and Kharel, Prashanta and Yoon, Taekwan and Frunzio, Luigi and Rakich, Peter T. and Schoelkopf, Robert J.},
	month = nov,
	year = {2018},
	pages = {666--670},
	file = {Full Text PDF:C\:\\Users\\abarbero\\Zotero\\storage\\T6E8MZB4\\Chu et al. - 2018 - Creation and control of multi-phonon Fock states in a bulk acoustic-wave resonator.pdf:application/pdf},
}

@article{maccabe_nano-acoustic_2020,
	title = {Nano-acoustic resonator with ultralong phonon lifetime},
	volume = {370},
	url = {https://www.science.org/doi/10.1126/science.abc7312},
	doi = {10.1126/science.abc7312},
	abstract = {The energy damping time in a mechanical resonator is critical to many precision metrology applications, such as timekeeping and force measurements. We present measurements of the phonon lifetime of a microwave-frequency, nanoscale silicon acoustic cavity incorporating a phononic bandgap acoustic shield. Using pulsed laser light to excite a colocalized optical mode of the cavity, we measured the internal acoustic modes with single-phonon sensitivity down to millikelvin temperatures, yielding a phonon lifetime of up to 
τph,0≈1.5
 seconds (quality factor 
Q=5×1010
) and a coherence time of 
τcoh,0≈130
 microseconds for bandgap-shielded cavities. These acoustically engineered nanoscale structures provide a window into the material origins of quantum noise and have potential applications ranging from tests of various collapse models of quantum mechanics to miniature quantum memory elements in hybrid superconducting quantum circuits.},
	number = {6518},
	urldate = {2024-12-02},
	journal = {Science},
	author = {MacCabe, Gregory S. and Ren, Hengjiang and Luo, Jie and Cohen, Justin D. and Zhou, Hengyun and Sipahigil, Alp and Mirhosseini, Mohammad and Painter, Oskar},
	month = nov,
	year = {2020},
	pages = {840--843},
	file = {Version acceptée:C\:\\Users\\abarbero\\Zotero\\storage\\YD88Q2JZ\\MacCabe et al. - 2020 - Nano-acoustic resonator with ultralong phonon life.pdf:application/pdf},
}

@article{vainsencher_bi-directional_2016,
	title = {Bi-directional conversion between microwave and optical frequencies in a piezoelectric optomechanical device},
	volume = {109},
	issn = {0003-6951},
	url = {https://doi.org/10.1063/1.4955408},
	doi = {10.1063/1.4955408},
	abstract = {We describe the principles of design, fabrication, and operation of a piezoelectric optomechanical crystal with which we demonstrate bi-directional conversion of energy between microwave and optical frequencies. The optomechanical crystal has an optical mode at 1523 nm co-located with a mechanical breathing mode at 3.8 GHz, with a measured optomechanical coupling strength gom/2π of 115 kHz. The breathing mode is driven and detected by curved interdigitated transducers that couple to a Lamb mode in suspended membranes on either end of the optomechanical crystal, allowing the external piezoelectric modulation of the optical signal as well as the converse, the detection of microwave electrical signals generated by a modulated optical signal. We compare measurements to theory where appropriate.},
	number = {3},
	urldate = {2025-08-04},
	journal = {Applied Physics Letters},
	author = {Vainsencher, Amit and Satzinger, K. J. and Peairs, G. A. and Cleland, A. N.},
	month = jul,
	year = {2016},
	pages = {033107},
	file = {Full Text PDF:C\:\\Users\\abarbero\\Zotero\\storage\\695I39Z3\\Vainsencher et al. - 2016 - Bi-directional conversion between microwave and optical frequencies in a piezoelectric optomechanica.pdf:application/pdf;Snapshot:C\:\\Users\\abarbero\\Zotero\\storage\\JNQDDCNZ\\1.html:text/html},
}

@article{kimble_quantum_2008,
	title = {The quantum internet},
	volume = {453},
	copyright = {2008 Springer Nature Limited},
	issn = {1476-4687},
	url = {https://www.nature.com/articles/nature07127},
	doi = {10.1038/nature07127},
	abstract = {Quantum networks provide opportunities and challenges across a range of intellectual and technical frontiers, including quantum computation, communication and metrology. The realization of quantum networks composed of many nodes and channels requires new scientific capabilities for generating and characterizing quantum coherence and entanglement. Fundamental to this endeavour are quantum interconnects, which convert quantum states from one physical system to those of another in a reversible manner. Such quantum connectivity in networks can be achieved by the optical interactions of single photons and atoms, allowing the distribution of entanglement across the network and the teleportation of quantum states between nodes.},
	language = {en},
	number = {7198},
	urldate = {2025-07-31},
	journal = {Nature},
	author = {Kimble, H. J.},
	month = jun,
	year = {2008},
	pages = {1023--1030},
	file = {Full Text PDF:C\:\\Users\\abarbero\\Zotero\\storage\\2VRN9I92\\Kimble - 2008 - The quantum internet.pdf:application/pdf},
}

@article{forsch_microwave--optics_2020,
	title = {Microwave-to-optics conversion using a mechanical oscillator in its quantum ground state},
	volume = {16},
	copyright = {2019 The Author(s), under exclusive licence to Springer Nature Limited},
	issn = {1745-2481},
	url = {https://www.nature.com/articles/s41567-019-0673-7},
	doi = {10.1038/s41567-019-0673-7},
	abstract = {Conversion between signals in the microwave and optical domains is of great interest both for classical telecommunication and for connecting future superconducting quantum computers into a global quantum network. For quantum applications, the conversion has to be efficient, as well as operate in a regime of minimal added classical noise. While efficient conversion has been demonstrated using mechanical transducers, they have so far all operated with a substantial thermal noise background. Here, we overcome this limitation and demonstrate coherent conversion between gigahertz microwave signals and the optical telecom band with a thermal background of less than one phonon. We use an integrated, on-chip electro-optomechanical device that couples surface acoustic waves driven by a resonant microwave signal to an optomechanical crystal featuring a 2.7 GHz mechanical mode. We initialize the mechanical mode in its quantum ground state, which allows us to perform the transduction process with minimal added thermal noise, while maintaining an optomechanical cooperativity {\textgreater}1, so that microwave photons mapped into the mechanical resonator are effectively upconverted to the optical domain. We further verify the preservation of the coherence of the microwave signal throughout the transduction process.},
	language = {en},
	number = {1},
	urldate = {2025-08-04},
	journal = {Nature Physics},
	author = {Forsch, Moritz and Stockill, Robert and Wallucks, Andreas and Marinković, Igor and Gärtner, Claus and Norte, Richard A. and van Otten, Frank and Fiore, Andrea and Srinivasan, Kartik and Gröblacher, Simon},
	month = jan,
	year = {2020},
	pages = {69--74},
	file = {Full Text PDF:C\:\\Users\\abarbero\\Zotero\\storage\\9FCMRQE3\\Forsch et al. - 2020 - Microwave-to-optics conversion using a mechanical oscillator in its quantum ground state.pdf:application/pdf},
}

@article{arnold_converting_2020,
	title = {Converting microwave and telecom photons with a silicon photonic nanomechanical interface},
	volume = {11},
	copyright = {2020 The Author(s)},
	issn = {2041-1723},
	url = {https://www.nature.com/articles/s41467-020-18269-z},
	doi = {10.1038/s41467-020-18269-z},
	abstract = {Practical quantum networks require low-loss and noise-resilient optical interconnects as well as non-Gaussian resources for entanglement distillation and distributed quantum computation. The latter could be provided by superconducting circuits but existing solutions to interface the microwave and optical domains lack either scalability or efficiency, and in most cases the conversion noise is not known. In this work we utilize the unique opportunities of silicon photonics, cavity optomechanics and superconducting circuits to demonstrate a fully integrated, coherent transducer interfacing the microwave X and the telecom S bands with a total (internal) bidirectional transduction efficiency of 1.2\% (135\%) at millikelvin temperatures. The coupling relies solely on the radiation pressure interaction mediated by the femtometer-scale motion of two silicon nanobeams reaching a Vπ as low as 16 μV for sub-nanowatt pump powers. Without the associated optomechanical gain, we achieve a total (internal) pure conversion efficiency of up to 0.019\% (1.6\%), relevant for future noise-free operation on this qubit-compatible platform.},
	language = {en},
	number = {1},
	urldate = {2025-08-04},
	journal = {Nature Communications},
	author = {Arnold, G. and Wulf, M. and Barzanjeh, S. and Redchenko, E. S. and Rueda, A. and Hease, W. J. and Hassani, F. and Fink, J. M.},
	month = sep,
	year = {2020},
	pages = {4460},
	file = {Full Text PDF:C\:\\Users\\abarbero\\Zotero\\storage\\2GDIPYIS\\Arnold et al. - 2020 - Converting microwave and telecom photons with a silicon photonic nanomechanical interface.pdf:application/pdf},
}

@article{mirhosseini_superconducting_2020,
	title = {Superconducting qubit to optical photon transduction},
	volume = {588},
	copyright = {2020 The Author(s), under exclusive licence to Springer Nature Limited},
	issn = {1476-4687},
	url = {https://www.nature.com/articles/s41586-020-3038-6},
	doi = {10.1038/s41586-020-3038-6},
	abstract = {Conversion of electrical and optical signals lies at the foundation of the global internet. Such converters are used to extend the reach of long-haul fibre-optic communication systems and within data centres for high-speed optical networking of computers. Likewise, coherent microwave-to-optical conversion of single photons would enable the exchange of quantum states between remotely connected superconducting quantum processors1. Despite the prospects of quantum networking2, maintaining the fragile quantum state in such a conversion process with superconducting qubits has not yet been achieved. Here we demonstrate the conversion of a microwave-frequency excitation of a transmon—a type of superconducting qubit—into an optical photon. We achieve this by using an intermediary nanomechanical resonator that converts the electrical excitation of the qubit into a single phonon by means of a piezoelectric interaction3 and subsequently converts the phonon to an optical photon by means of radiation pressure4. We demonstrate optical photon generation from the qubit by recording quantum Rabi oscillations of the qubit through single-photon detection of the emitted light over an optical fibre. With proposed improvements in the device and external measurement set-up, such quantum transducers might be used to realize new hybrid quantum networks2,5 and, ultimately, distributed quantum computers6,7.},
	language = {en},
	number = {7839},
	urldate = {2025-08-04},
	journal = {Nature},
	author = {Mirhosseini, Mohammad and Sipahigil, Alp and Kalaee, Mahmoud and Painter, Oskar},
	month = dec,
	year = {2020},
	pages = {599--603},
	file = {Full Text PDF:C\:\\Users\\abarbero\\Zotero\\storage\\7N56TQYR\\Mirhosseini et al. - 2020 - Superconducting qubit to optical photon transduction.pdf:application/pdf},
}

@article{honl_microwave--optical_2022,
	title = {Microwave-to-optical conversion with a gallium phosphide photonic crystal cavity},
	volume = {13},
	copyright = {2022 The Author(s)},
	issn = {2041-1723},
	url = {https://www.nature.com/articles/s41467-022-28670-5},
	doi = {10.1038/s41467-022-28670-5},
	abstract = {Electrically actuated optomechanical resonators provide a route to quantum-coherent, bidirectional conversion of microwave and optical photons. Such devices could enable optical interconnection of quantum computers based on qubits operating at microwave frequencies. Here we present a platform for microwave-to-optical conversion comprising a photonic crystal cavity made of single-crystal, piezoelectric gallium phosphide integrated on pre-fabricated niobium circuits on an intrinsic silicon substrate. The devices exploit spatially extended, sideband-resolved mechanical breathing modes at {\textasciitilde}3.2 GHz, with vacuum optomechanical coupling rates of up to g0/2π ≈ 300 kHz. The mechanical modes are driven by integrated microwave electrodes via the inverse piezoelectric effect. We estimate that the system could achieve an electromechanical coupling rate to a superconducting transmon qubit of {\textasciitilde}200 kHz. Our work represents a decisive step towards integration of piezoelectro-optomechanical interfaces with superconducting quantum processors.},
	language = {en},
	number = {1},
	urldate = {2025-08-05},
	journal = {Nature Communications},
	author = {Hönl, Simon and Popoff, Youri and Caimi, Daniele and Beccari, Alberto and Kippenberg, Tobias J. and Seidler, Paul},
	month = apr,
	year = {2022},
	pages = {2065},
	file = {Full Text PDF:C\:\\Users\\abarbero\\Zotero\\storage\\PYALCAHB\\Hönl et al. - 2022 - Microwave-to-optical conversion with a gallium phosphide photonic crystal cavity.pdf:application/pdf},
}

@article{jiang_optically_2023,
	title = {Optically heralded microwave photon addition},
	volume = {19},
	copyright = {2023 The Author(s), under exclusive licence to Springer Nature Limited},
	issn = {1745-2481},
	url = {https://www.nature.com/articles/s41567-023-02129-w},
	doi = {10.1038/s41567-023-02129-w},
	abstract = {Photons with optical frequencies of a few hundred terahertz are perhaps the only way to distribute quantum information over long distances. Superconducting qubits, which are one of the most promising approaches for realizing large-scale quantum machines, operate on microwave photons at frequencies that are {\textasciitilde}40,000 times lower. To network these quantum machines across appreciable distances, we must bridge this frequency gap. Here we implement and demonstrate a transducer that can generate correlated optical and microwave photons. We use it to show that by detecting an optical photon we generate an added microwave photon with an efficiency of {\textasciitilde}35\%. Our device uses a gigahertz nanomechanical resonance as an intermediary, which efficiently couples to optical and microwave channels through strong optomechanical and piezoelectric interactions. We show continuous operation of the transducer with 5\% frequency conversion efficiency, input-referred added noise of {\textasciitilde}100, and pulsed microwave photon generation at a heralding rate of 15 Hz. Optical absorption in the device generates thermal noise of less than two microwave photons. Improvements of the system efficiencies and device performance are necessary to realize a high rate of entanglement generation between distant microwave-frequency quantum nodes, but these enhancements are within reach.},
	language = {en},
	number = {10},
	urldate = {2025-08-04},
	journal = {Nature Physics},
	author = {Jiang, Wentao and Mayor, Felix M. and Malik, Sultan and Van Laer, Raphaël and McKenna, Timothy P. and Patel, Rishi N. and Witmer, Jeremy D. and Safavi-Naeini, Amir H.},
	month = oct,
	year = {2023},
	pages = {1423--1428},
	file = {Full Text PDF:C\:\\Users\\abarbero\\Zotero\\storage\\NW3JZPWU\\Jiang et al. - 2023 - Optically heralded microwave photon addition.pdf:application/pdf},
}

@article{meesala_non-classical_2024,
	title = {Non-classical microwave–optical photon pair generation with a chip-scale transducer},
	volume = {20},
	copyright = {2024 The Author(s), under exclusive licence to Springer Nature Limited},
	issn = {1745-2481},
	url = {https://www.nature.com/articles/s41567-024-02409-z},
	doi = {10.1038/s41567-024-02409-z},
	abstract = {Modern computing and communication technologies such as supercomputers and the Internet are based on optically connected networks of microwave-frequency information processors. An analogous architecture has been proposed for quantum networks, using optical photons to distribute entanglement between remote superconducting quantum processors. Here we report a step towards such a network by observing non-classical correlations between photons in an optical link and a superconducting quantum device. We generate these states of light through a spontaneous parametric down-conversion process in a chip-scale piezo-optomechanical transducer, and we measure a microwave–optical cross-correlation exceeding the Cauchy–Schwarz classical bound for thermal states. As further evidence of the non-classical character of the microwave–optical photon pairs, we observe antibunching in the microwave state conditioned on detection of an optical photon. Such a transducer can be readily connected to an independent superconducting qubit module and serve as a key building block for optical quantum networks of microwave-frequency qubits.},
	language = {en},
	number = {5},
	urldate = {2025-08-04},
	journal = {Nature Physics},
	author = {Meesala, Srujan and Wood, Steven and Lake, David and Chiappina, Piero and Zhong, Changchun and Beyer, Andrew D. and Shaw, Matthew D. and Jiang, Liang and Painter, Oskar},
	month = may,
	year = {2024},
	pages = {871--877},
	file = {Full Text PDF:C\:\\Users\\abarbero\\Zotero\\storage\\SD7MY44G\\Meesala et al. - 2024 - Non-classical microwave–optical photon pair generation with a chip-scale transducer.pdf:application/pdf},
}

@article{blesin_bidirectional_2024,
	title = {Bidirectional microwave-optical transduction based on integration of high-overtone bulk acoustic resonators and photonic circuits},
	volume = {15},
	copyright = {2024 The Author(s)},
	issn = {2041-1723},
	url = {https://www.nature.com/articles/s41467-024-49467-8},
	doi = {10.1038/s41467-024-49467-8},
	abstract = {Coherent interconversion between microwave and optical frequencies can serve as both classical and quantum interfaces for computing, communication, and sensing. Here, we present a compact microwave-optical transducer based on monolithic integration of piezoelectric actuators on silicon nitride photonic circuits. Such an actuator couples microwave signals to a high-overtone bulk acoustic resonator defined by the silica cladding of the optical waveguide core, suspended to enhance electromechanical and optomechanical couplings. At room temperature, this triply resonant piezo-optomechanical transducer achieves an off-chip photon number conversion efficiency of 1.6 × 10−5 over a bandwidth of 25 MHz at an input pump power of 21 dBm. The approach is scalable in manufacturing and does not rely on superconducting resonators. As the transduction process is bidirectional, we further demonstrate the synthesis of microwave pulses from a purely optical input. Capable of leveraging multiple acoustic modes for transduction, this platform offers prospects for frequency-multiplexed qubit interconnects and microwave photonics at large.},
	language = {en},
	number = {1},
	urldate = {2025-08-05},
	journal = {Nature Communications},
	author = {Blésin, Terence and Kao, Wil and Siddharth, Anat and Wang, Rui N. and Attanasio, Alaina and Tian, Hao and Bhave, Sunil A. and Kippenberg, Tobias J.},
	month = jul,
	year = {2024},
	pages = {6096},
	file = {Full Text PDF:C\:\\Users\\abarbero\\Zotero\\storage\\68X76CQX\\Blésin et al. - 2024 - Bidirectional microwave-optical transduction based on integration of high-overtone bulk acoustic res.pdf:application/pdf},
}

@article{van_thiel_optical_2025,
	title = {Optical readout of a superconducting qubit using a piezo-optomechanical transducer},
	volume = {21},
	copyright = {2025 The Author(s), under exclusive licence to Springer Nature Limited},
	issn = {1745-2481},
	url = {https://www.nature.com/articles/s41567-024-02742-3},
	doi = {10.1038/s41567-024-02742-3},
	abstract = {Superconducting quantum processors have made important progress in size and computing potential. However, the practical cryogenic limitations of operating large numbers of superconducting qubits are becoming a bottleneck for further scaling. Due to the low thermal conductivity and the dense optical multiplexing capacity of telecommunications fibre, converting qubit signal processing to the optical domain using microwave-to-optics transduction would substantially relax the strain on cryogenic space and thermal budgets. Here we demonstrate optical readout of a superconducting transmon qubit through an optical fibre connected via a coaxial cable to a fully integrated piezo-optomechanical transducer. Using a demolition readout technique, we achieve a single-shot readout fidelity of 81\%. Our results illustrate the benefits of piezo-optomechanical transduction for low-dissipation operation of large quantum processors.},
	language = {en},
	number = {3},
	urldate = {2025-08-04},
	journal = {Nature Physics},
	author = {van Thiel, T. C. and Weaver, M. J. and Berto, F. and Duivestein, P. and Lemang, M. and Schuurman, K. L. and Žemlička, M. and Hijazi, F. and Bernasconi, A. C. and Ferrer, C. and Cataldo, E. and Lachman, E. and Field, M. and Mohan, Y. and de Vries, F. K. and Bultink, C. C. and van Oven, J. C. and Mutus, J. Y. and Stockill, R. and Gröblacher, S.},
	month = mar,
	year = {2025},
	pages = {401--405},
}

@article{brubaker_optomechanical_2022,
	title = {Optomechanical {Ground}-{State} {Cooling} in a {Continuous} and {Efficient} {Electro}-{Optic} {Transducer}},
	volume = {12},
	url = {https://link.aps.org/doi/10.1103/PhysRevX.12.021062},
	doi = {10.1103/PhysRevX.12.021062},
	abstract = {The demonstration of a quantum link between microwave and optical frequencies would be an important step toward the realization of a quantum network of superconducting processors. A major impediment to quantum electro-optic transduction in all platforms explored to date is noise added by thermal occupation of modes involved in the transduction process, and it has proved difficult to realize low thermal occupancy concurrently with other desirable features like high duty cycle and high efficiency. In this work, we present an efficient and continuously operating electro-optomechanical transducer whose mechanical mode has been optically sideband cooled to its quantum ground state. The transducer achieves a maximum efficiency of 47\% and minimum input-referred added noise of 3.2 photons in upconversion. Moreover, the thermal occupancy of the transducer’s microwave mode is minimally affected by continuous laser illumination with power more than 2 orders of magnitude greater than that required for optomechanical ground-state cooling.},
	number = {2},
	urldate = {2025-08-04},
	journal = {Physical Review X},
	author = {Brubaker, B. M. and Kindem, J. M. and Urmey, M. D. and Mittal, S. and Delaney, R. D. and Burns, P. S. and Vissers, M. R. and Lehnert, K. W. and Regal, C. A.},
	month = jun,
	year = {2022},
	pages = {021062},
	file = {APS Snapshot:C\:\\Users\\abarbero\\Zotero\\storage\\WU9QHP26\\PhysRevX.12.html:text/html;Full Text PDF:C\:\\Users\\abarbero\\Zotero\\storage\\5UJU6VR2\\Brubaker et al. - 2022 - Optomechanical Ground-State Cooling in a Continuous and Efficient Electro-Optic Transducer.pdf:application/pdf},
}

@article{zhao_quantum-enabled_2025,
	title = {Quantum-enabled microwave-to-optical transduction via silicon nanomechanics},
	volume = {20},
	copyright = {2025 The Author(s), under exclusive licence to Springer Nature Limited},
	issn = {1748-3395},
	url = {https://www.nature.com/articles/s41565-025-01874-8},
	doi = {10.1038/s41565-025-01874-8},
	abstract = {An interface between microwave and optical photons offers the potential to network remote superconducting quantum processors. To preserve fragile quantum states, a microwave-to-optical transducer must operate efficiently in the quantum-enabled regime by generating less than one photon of noise referred to its input. Here we achieve these criteria using an integrated electro-optomechanical device made from crystalline silicon. Our platform eliminates the need for heterogeneous integration with piezoelectric materials by utilizing electrostatic actuation of gigahertz-frequency nanomechanical oscillators. Leveraging the ultra-low mechanical dissipation in silicon, our microwave-to-optical transducers achieve below one photon of input-referred added noise (nadd = 0.58) under continuous-wave laser drives. This demonstration of continuous quantum-enabled microwave-to-optical transduction improves the upconversion rate by about two orders of magnitude beyond the state of the art (R = 0.47–1.9 kHz). The increased transduction rate and scalable fabrication of our devices may facilitate near-term use of transducers in distributed quantum computers and quantum networks.},
	language = {en},
	number = {5},
	urldate = {2025-08-04},
	journal = {Nature Nanotechnology},
	author = {Zhao, Han and Chen, William David and Kejriwal, Abhishek and Mirhosseini, Mohammad},
	month = may,
	year = {2025},
	pages = {602--608},
	file = {Full Text PDF:C\:\\Users\\abarbero\\Zotero\\storage\\Q5KDRUNB\\Zhao et al. - 2025 - Quantum-enabled microwave-to-optical transduction via silicon nanomechanics.pdf:application/pdf},
}

@article{bagci_optical_2014,
	title = {Optical detection of radio waves through a nanomechanical transducer},
	volume = {507},
	copyright = {2014 Springer Nature Limited},
	issn = {1476-4687},
	url = {https://www.nature.com/articles/nature13029},
	doi = {10.1038/nature13029},
	abstract = {A room-temperature nanomechanical transducer that couples efficiently to both radio waves and light allows radio-frequency signals to be detected as an optical phase shift with quantum-limited sensitivity.},
	language = {en},
	number = {7490},
	urldate = {2025-10-07},
	journal = {Nature},
	author = {Bagci, T. and Simonsen, A. and Schmid, S. and Villanueva, L. G. and Zeuthen, E. and Appel, J. and Taylor, J. M. and Sørensen, A. and Usami, K. and Schliesser, A. and Polzik, E. S.},
	month = mar,
	year = {2014},
	pages = {81--85},
}

@article{halg_membrane-based_2021,
	title = {Membrane-{Based} {Scanning} {Force} {Microscopy}},
	volume = {15},
	url = {https://link.aps.org/doi/10.1103/PhysRevApplied.15.L021001},
	doi = {10.1103/PhysRevApplied.15.L021001},
	abstract = {We report the development of a scanning force microscope based on an ultrasensitive silicon nitride membrane optomechanical transducer. Our development is made possible by inverting the standard microscope geometry—in our instrument, the substrate is vibrating and the scanning tip is at rest. We present topography images of samples placed on the membrane surface. Our measurements demonstrate that the membrane retains an excellent force sensitivity when loaded with samples and in the presence of a scanning tip. We discuss the prospects and limitations of our instrument as a quantum-limited force sensor and imaging tool.},
	number = {2},
	urldate = {2025-10-07},
	journal = {Physical Review Applied},
	author = {Hälg, David and Gisler, Thomas and Tsaturyan, Yeghishe and Catalini, Letizia and Grob, Urs and Krass, Marc-Dominik and Héritier, Martin and Mattiat, Hinrich and Thamm, Ann-Katrin and Schirhagl, Romana and Langman, Eric C. and Schliesser, Albert and Degen, Christian L. and Eichler, Alexander},
	month = feb,
	year = {2021},
	pages = {L021001},
	file = {APS Snapshot:C\:\\Users\\abarbero\\Zotero\\storage\\59NAKW5M\\PhysRevApplied.15.html:text/html;Full Text PDF:C\:\\Users\\abarbero\\Zotero\\storage\\5B43PHBK\\Hälg et al. - 2021 - Membrane-Based Scanning Force Microscopy.pdf:application/pdf},
}

@article{chowdhury_membrane-based_2023,
	title = {Membrane-{Based} {Optomechanical} {Accelerometry}},
	volume = {19},
	url = {https://link.aps.org/doi/10.1103/PhysRevApplied.19.024011},
	doi = {10.1103/PhysRevApplied.19.024011},
	abstract = {Optomechanical accelerometers promise quantum-limited readout, high detection bandwidth, self-calibration, and radiation-pressure stabilization. We present a simple, scalable platform that enables these benefits with nano-�� sensitivity at acoustic frequencies, based on a pair of vertically integrated Si3⁢N4 membranes with different stiffnesses, forming an optical cavity. As a demonstration, we integrate an ultrahigh-�� ( {\textgreater}107), millimeter-scale Si3⁢N4 trampoline membrane above an unpatterned membrane on the same Si chip, forming a finesse ℱ ≈2 cavity. Using direct photodetection in transmission, we resolve the relative displacement of the membranes with a shot-noise-limited imprecision of 7 fm/√Hz, yielding a thermal-noise-limited acceleration sensitivity of 0.6 ��⁢g⁡/√Hz over a 1-kHz bandwidth centered on the fundamental trampoline resonance (40 kHz). To illustrate the advantage of radiation-pressure stabilization, we cold damp the trampoline to an effective temperature of 4 mK and leverage the reduced energy variance to resolve an applied stochastic acceleration of 50 ng/√Hz in an integration time of minutes. In the future, we envision a small-scale array of these devices operating in a cryostat to search for fundamental weak forces such as dark matter.},
	number = {2},
	urldate = {2025-10-07},
	journal = {Physical Review Applied},
	author = {Chowdhury, Mitul Dey and Agrawal, Aman R. and Wilson, Dalziel J.},
	month = feb,
	year = {2023},
	pages = {024011},
	file = {APS Snapshot:C\:\\Users\\abarbero\\Zotero\\storage\\ZBHMIXQB\\PhysRevApplied.19.html:text/html;Full Text PDF:C\:\\Users\\abarbero\\Zotero\\storage\\ESTPZ9JH\\Chowdhury et al. - 2023 - Membrane-Based Optomechanical Accelerometry.pdf:application/pdf},
}

@article{salimi_squeeze_2024,
	title = {Squeeze film absolute pressure sensors with sub-millipascal sensitivity},
	volume = {374},
	issn = {0924-4247},
	url = {https://www.sciencedirect.com/science/article/pii/S0924424724004448},
	doi = {10.1016/j.sna.2024.115450},
	abstract = {We report on the realization of ultrasensitive absolute pressure sensors based on silicon nitride membrane sandwiches. These sandwiches consist in a pair of highly-pretensioned, ultrathin (50 nm), large area (0.25 mm2) films, suspended parallel to each other and forming an ultrashort (500 nm) open cavity. The compression of a gas in this cavity leads to a strong squeeze film force, resulting in an increase in the membrane mechanical resonance frequencies, which is directly proportional to the absolute gas pressure. These sandwiches show a record high responsivity of {\textgreater}300 Hz/Pa in terms of squeeze film-induced frequency shift in the range 10−3-100 Pa, which, combined with high quality factor mechanical resonances (Q{\textgreater}106), allows for bringing the sensitivity of absolute squeeze film pressure sensors down to the sub-millipascal level.},
	urldate = {2025-10-07},
	journal = {Sensors and Actuators A: Physical},
	author = {Salimi, Mohsen and Nielsen, Robin V. and Pedersen, Henrik B. and Dantan, Aurélien},
	month = aug,
	year = {2024},
	pages = {115450},
	file = {ScienceDirect Full Text PDF:C\:\\Users\\abarbero\\Zotero\\storage\\ET9LFRV4\\Salimi et al. - 2024 - Squeeze film absolute pressure sensors with sub-millipascal sensitivity.pdf:application/pdf;ScienceDirect Snapshot:C\:\\Users\\abarbero\\Zotero\\storage\\SKSC2TYG\\S0924424724004448.html:text/html},
}

@article{doeleman_brillouin_2023,
	title = {Brillouin optomechanics in the quantum ground state},
	volume = {5},
	url = {https://link.aps.org/doi/10.1103/PhysRevResearch.5.043140},
	doi = {10.1103/PhysRevResearch.5.043140},
	abstract = {Bulk acoustic wave (BAW) resonators are attractive as intermediaries in a microwave-to-optical transducer, due to their long coherence times and controllable coupling to optical photons and superconducting qubits. However, for an optomechanical transducer to operate without detrimental added noise, the mechanical modes must be in the quantum ground state. This has proven challenging in recent demonstrations of transduction based on other types of mechanical resonators, where absorption of laser light caused heating of the phonon modes. In this work, we demonstrate ground-state operation of a Brillouin optomechanical system composed of a quartz BAW resonator inside an optical cavity. We show optomechanical coupling to several phonon modes and perform sideband asymmetry thermometry to demonstrate a thermal occupation below 0.5 phonons at base temperature. This constitutes the heaviest (∼494µ⁢g) mechanical object measured in the quantum ground state to date. Further measurements confirm a negligible effect of laser heating on this phonon occupation. Our results pave the way toward low-noise, high-efficiency microwave-to-optical transduction based on BAW resonators.},
	number = {4},
	urldate = {2025-08-05},
	journal = {Physical Review Research},
	author = {Doeleman, H. M. and Schatteburg, T. and Benevides, R. and Vollenweider, S. and Macri, D. and Chu, Y.},
	month = nov,
	year = {2023},
	pages = {043140},
	file = {APS Snapshot:C\:\\Users\\abarbero\\Zotero\\storage\\KJT3YEGF\\PhysRevResearch.5.html:text/html;Full Text PDF:C\:\\Users\\abarbero\\Zotero\\storage\\PKUSQ5X5\\Doeleman et al. - 2023 - Brillouin optomechanics in the quantum ground state.pdf:application/pdf},
}

@article{cattiaux_macroscopic_2021,
	title = {A macroscopic object passively cooled into its quantum ground state of motion beyond single-mode cooling},
	volume = {12},
	copyright = {2021 The Author(s)},
	issn = {2041-1723},
	url = {https://www.nature.com/articles/s41467-021-26457-8},
	doi = {10.1038/s41467-021-26457-8},
	abstract = {The nature of the quantum-to-classical crossover remains one of the most challenging open question of Science to date. In this respect, moving objects play a specific role. Pioneering experiments over the last few years have begun exploring quantum behaviour of micron-sized mechanical systems, either by passively cooling single GHz modes, or by adapting laser cooling techniques developed in atomic physics to cool specific low-frequency modes far below the temperature of their surroundings. Here instead we describe a very different approach, passive cooling of a whole micromechanical system down to 500 μK, reducing the average number of quanta in the fundamental vibrational mode at 15 MHz to just 0.3 (with even lower values expected for higher harmonics); the challenge being to be still able to detect the motion without disturbing the system noticeably. With such an approach higher harmonics and the surrounding environment are also cooled, leading to potentially much longer mechanical coherence times, and enabling experiments questioning mechanical wave-function collapse, potentially from the gravitational background, and quantum thermodynamics. Beyond the average behaviour, here we also report on the fluctuations of the fundamental vibrational mode of the device in-equilibrium with the cryostat. These reveal a surprisingly complex interplay with the local environment and allow characteristics of two distinct thermodynamic baths to be probed.},
	language = {en},
	number = {1},
	urldate = {2025-08-05},
	journal = {Nature Communications},
	author = {Cattiaux, D. and Golokolenov, I. and Kumar, S. and Sillanpää, M. and Mercier de Lépinay, L. and Gazizulin, R. R. and Zhou, X. and Armour, A. D. and Bourgeois, O. and Fefferman, A. and Collin, E.},
	month = oct,
	year = {2021},
	pages = {6182},
	file = {Full Text PDF:C\:\\Users\\abarbero\\Zotero\\storage\\69F7C975\\Cattiaux et al. - 2021 - A macroscopic object passively cooled into its quantum ground state of motion beyond single-mode coo.pdf:application/pdf},
}

@article{galinskiy_phonon_2020,
	title = {Phonon counting thermometry of an ultracoherent membrane resonator near its motional ground state},
	volume = {7},
	copyright = {© 2020 Optical Society of America},
	issn = {2334-2536},
	url = {https://opg.optica.org/optica/abstract.cfm?uri=optica-7-6-718},
	doi = {10.1364/OPTICA.390939},
	abstract = {The generation of non-Gaussian quantum states of macroscopic mechanical objects is key to a number of challenges in quantum information science, ranging from fundamental tests of decoherence to quantum communication and sensing. Heralded generation of single-phonon states of mechanical motion is an attractive way toward this goal, as it is, in principle, not limited by the object size. Here we demonstrate a technique that allows for generation and detection of a quantum state of motion by phonon counting measurements near the ground state of a 1.5 MHz micromechanical oscillator. We detect scattered photons from a membrane-in-the-middle optomechanical system using an ultra-narrowband optical filter, and perform Raman-ratio thermometry and second-order intensity interferometry near the motional ground state (n¯=0.23±0.02phonons). With an effective mass in the nanogram range, our system lends itself for studies of long-lived non-Gaussian motional states with some of the heaviest objects to date.},
	language = {EN},
	number = {6},
	urldate = {2025-08-05},
	journal = {Optica},
	author = {Galinskiy, I. and Tsaturyan, Y. and Parniak, M. and Polzik, E. S.},
	month = jun,
	year = {2020},
	pages = {718--725},
	file = {Full Text PDF:C\:\\Users\\abarbero\\Zotero\\storage\\5DMYXWJF\\Galinskiy et al. - 2020 - Phonon counting thermometry of an ultracoherent membrane resonator near its motional ground state.pdf:application/pdf},
}

@article{patil_measuring_2022,
	title = {Measuring {High}-{Order} {Phonon} {Correlations} in an {Optomechanical} {Resonator}},
	volume = {128},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.128.183601},
	doi = {10.1103/PhysRevLett.128.183601},
	abstract = {We use single photon detectors to probe the motional state of a superfluid 4He resonator of mass ∼1 ng. The arrival times of Stokes and anti-Stokes photons (scattered by the resonator’s acoustic mode) are used to measure the resonator’s phonon coherences up to the fourth order. By postselecting on photon detection events, we also measure coherences in the resonator when ≤3 phonons have been added or subtracted. These measurements are found to be consistent with predictions that assume the acoustic mode to be in thermal equilibrium with a bath through a Markovian coupling.},
	number = {18},
	urldate = {2025-08-05},
	journal = {Physical Review Letters},
	author = {Patil, Y. S. S. and Yu, J. and Frazier, S. and Wang, Y. and Johnson, K. and Fox, J. and Reichel, J. and Harris, J. G. E.},
	month = may,
	year = {2022},
	pages = {183601},
	file = {APS Snapshot:C\:\\Users\\abarbero\\Zotero\\storage\\TBQNGVFH\\PhysRevLett.128.html:text/html;Version acceptée:C\:\\Users\\abarbero\\Zotero\\storage\\2ZYFYETG\\Patil et al. - 2022 - Measuring High-Order Phonon Correlations in an Optomechanical Resonator.pdf:application/pdf},
}

@article{delic_cooling_2020,
	title = {Cooling of a levitated nanoparticle to the motional quantum ground state},
	volume = {367},
	url = {https://www.science.org/doi/10.1126/science.aba3993},
	doi = {10.1126/science.aba3993},
	abstract = {Quantum control of complex objects in the regime of large size and mass provides opportunities for sensing applications and tests of fundamental physics. The realization of such extreme quantum states of matter remains a major challenge. We demonstrate a quantum interface that combines optical trapping of solids with cavity-mediated light-matter interaction. Precise control over the frequency and position of the trap laser with respect to the optical cavity allowed us to laser-cool an optically trapped nanoparticle into its quantum ground state of motion from room temperature. The particle comprises 108 atoms, similar to current Bose-Einstein condensates, with the density of a solid object. Our cooling technique, in combination with optical trap manipulation, may enable otherwise unachievable superposition states involving large masses.},
	number = {6480},
	urldate = {2025-08-05},
	journal = {Science},
	author = {Delić, Uroš and Reisenbauer, Manuel and Dare, Kahan and Grass, David and Vuletić, Vladan and Kiesel, Nikolai and Aspelmeyer, Markus},
	month = feb,
	year = {2020},
	pages = {892--895},
	file = {Full Text PDF:C\:\\Users\\abarbero\\Zotero\\storage\\CUC6GM6F\\Delić et al. - 2020 - Cooling of a levitated nanoparticle to the motional quantum ground state.pdf:application/pdf},
}

@article{qiu_laser_2020,
	title = {Laser {Cooling} of a {Nanomechanical} {Oscillator} to {Its} {Zero}-{Point} {Energy}},
	volume = {124},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.124.173601},
	doi = {10.1103/PhysRevLett.124.173601},
	abstract = {Optomechanical systems in the well-resolved-sideband regime are ideal for studying a myriad of quantum phenomena with mechanical systems, including backaction-evading measurements, mechanical squeezing, and nonclassical states generation. For these experiments, the mechanical oscillator should be prepared in its ground state, i.e., exhibit negligible residual excess motion compared to its zero-point motion. This can be achieved using the radiation pressure of laser light in the cavity by selectively driving the lower motional sideband, leading to sideband cooling. To date, the preparation of sideband-resolved optical systems to their zero-point energy has eluded laser cooling because of strong optical absorption heating. The alternative method of passive cooling suffers from the same problem, as the requisite milliKelvin environment is incompatible with the strong optical driving needed by many quantum protocols. Here, we employ a highly sideband-resolved silicon optomechanical crystal in a 3He buffer-gas environment at ∼2 K to demonstrate laser sideband cooling to a mean thermal phonon occupancy of 0.09+0.02−0.01 quantum (self-calibrated using motional sideband asymmetry), which is −7.4 dB of the oscillator’s zero-point energy and corresponds to 92\% ground state probability. Achieving such low occupancy by laser cooling opens the door to a wide range of quantum-optomechanical experiments in the optical domain.},
	number = {17},
	urldate = {2025-08-05},
	journal = {Physical Review Letters},
	author = {Qiu, Liu and Shomroni, Itay and Seidler, Paul and Kippenberg, Tobias J.},
	month = apr,
	year = {2020},
	pages = {173601},
	file = {APS Snapshot:C\:\\Users\\abarbero\\Zotero\\storage\\D2TVE8VU\\PhysRevLett.124.html:text/html;Full Text PDF:C\:\\Users\\abarbero\\Zotero\\storage\\SUAFS8Y3\\Qiu et al. - 2020 - Laser Cooling of a Nanomechanical Oscillator to Its Zero-Point Energy.pdf:application/pdf},
}

@article{ramp_elimination_2019,
	title = {Elimination of {Thermomechanical} {Noise} in {Piezoelectric} {Optomechanical} {Crystals}},
	volume = {123},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.123.093603},
	doi = {10.1103/PhysRevLett.123.093603},
	abstract = {Mechanical modes are a potentially useful resource for quantum information applications, such as quantum-level wavelength transducers, due to their ability to interact with electromagnetic radiation across the spectrum. A significant challenge for wavelength transducers is thermomechanical noise in the mechanical mode, which pollutes the transduced signal with thermal states. In this Letter, we eliminate thermomechanical noise in the GHz-frequency mechanical breathing mode of a piezoelectric optomechanical crystal using cryogenic cooling in a dilution refrigerator. We optically measure an average thermal occupancy of the mechanical mode of only 0.7±0.4 phonons, providing a path towards low-noise microwave-to-optical conversion in the quantum regime.},
	number = {9},
	urldate = {2025-08-05},
	journal = {Physical Review Letters},
	author = {Ramp, H. and Hauer, B. D. and Balram, K. C. and Clark, T. J. and Srinivasan, K. and Davis, J. P.},
	month = aug,
	year = {2019},
	pages = {093603},
	file = {APS Snapshot:C\:\\Users\\abarbero\\Zotero\\storage\\KMMGXQR5\\PhysRevLett.123.html:text/html;Full Text PDF:C\:\\Users\\abarbero\\Zotero\\storage\\8SAUQ8ES\\Ramp et al. - 2019 - Elimination of Thermomechanical Noise in Piezoelectric Optomechanical Crystals.pdf:application/pdf},
}

@article{noguchi_ground_2016,
	title = {Ground state cooling of a quantum electromechanical system with a silicon nitride membrane in a {3D} loop-gap cavity},
	volume = {18},
	issn = {1367-2630},
	url = {https://dx.doi.org/10.1088/1367-2630/18/10/103036},
	doi = {10.1088/1367-2630/18/10/103036},
	abstract = {Cavity electro-(opto-)mechanics gives us a quantum tool to access mechanical modes in a massive object. Here we develop a quantum electromechanical system in which a vibrational mode of a SiNx membrane are coupled to a three-dimensional loop-gap superconducting microwave cavity. The tight confinement of the electric field across a mechanically compliant narrow-gap capacitor realizes the quantum strong coupling regime under a red-sideband pump field and the quantum ground state cooling of the mechanical mode. We also demonstrate strong coupling between two mechanical modes, which is induced by two-tone parametric drives and mediated by a virtual photon in the cavity.},
	language = {en},
	number = {10},
	urldate = {2025-08-05},
	journal = {New Journal of Physics},
	author = {Noguchi, Atsushi and Yamazaki, Rekishu and Ataka, Manabu and Fujita, Hiroyuki and Tabuchi, Yutaka and Ishikawa, Toyofumi and Usami, Koji and Nakamura, Yasunobu},
	month = oct,
	year = {2016},
	pages = {103036},
	file = {IOP Full Text PDF:C\:\\Users\\abarbero\\Zotero\\storage\\I22E2EUN\\Noguchi et al. - 2016 - Ground state cooling of a quantum electromechanical system with a silicon nitride membrane in a 3D l.pdf:application/pdf},
}

@article{chu_quantum_2017,
	title = {Quantum acoustics with superconducting qubits},
	volume = {358},
	url = {https://www.science.org/doi/10.1126/science.aao1511},
	doi = {10.1126/science.aao1511},
	abstract = {Mechanical objects have important practical applications in the fields of quantum information and metrology as quantum memories or transducers for measuring and connecting different types of quantum systems. The field of electromechanics is in pursuit of a robust and highly coherent device that couples motion to nonlinear quantum objects such as superconducting qubits. Here, we experimentally demonstrate a high-frequency bulk acoustic wave resonator that is strongly coupled to a superconducting qubit using piezoelectric transduction with a cooperativity of 260. We measure qubit and mechanical coherence times on the order of 10 microseconds. Our device requires only simple fabrication methods and provides controllable access to a multitude of phonon modes. We demonstrate quantum control and measurement on gigahertz phonons at the single-quantum level.},
	number = {6360},
	urldate = {2025-08-05},
	journal = {Science},
	author = {Chu, Yiwen and Kharel, Prashanta and Renninger, William H. and Burkhart, Luke D. and Frunzio, Luigi and Rakich, Peter T. and Schoelkopf, Robert J.},
	month = oct,
	year = {2017},
	pages = {199--202},
	file = {Full Text PDF:C\:\\Users\\abarbero\\Zotero\\storage\\RDNHNF3X\\Chu et al. - 2017 - Quantum acoustics with superconducting qubits.pdf:application/pdf},
}

@article{arrangoiz-arriola_resolving_2019,
	title = {Resolving the energy levels of a nanomechanical oscillator},
	volume = {571},
	copyright = {2019 The Author(s), under exclusive licence to Springer Nature Limited},
	issn = {1476-4687},
	url = {https://www.nature.com/articles/s41586-019-1386-x},
	doi = {10.1038/s41586-019-1386-x},
	abstract = {The quantum nature of an oscillating mechanical object is anything but apparent. The coherent states that describe the classical motion of a mechanical oscillator do not have a well defined energy, but are quantum superpositions of equally spaced energy eigenstates. Revealing this quantized structure is only possible with an apparatus that measures energy with a precision greater than the energy of a single phonon. One way to achieve this sensitivity is by engineering a strong but nonresonant interaction between the oscillator and an atom. In a system with sufficient quantum coherence, this interaction allows one to distinguish different energy eigenstates using resolvable differences in the atom’s transition frequency. For photons, such dispersive measurements have been performed in cavity1,2 and circuit quantum electrodynamics3. Here we report an experiment in which an artificial atom senses the motional energy of a driven nanomechanical oscillator with sufficient sensitivity to resolve the quantization of its energy. To realize this, we build a hybrid platform that integrates nanomechanical piezoelectric resonators with a microwave superconducting qubit on the same chip. We excite phonons with resonant pulses and probe the resulting excitation spectrum of the qubit to observe phonon-number-dependent frequency shifts that are about five times larger than the qubit linewidth. Our result demonstrates a fully integrated platform for quantum acoustics that combines large couplings, considerable coherence times and excellent control over the mechanical mode structure. With modest experimental improvements, we expect that our approach will enable quantum nondemolition measurements of phonons4 and will lead to quantum sensors and information-processing approaches5 that use chip-scale nanomechanical devices.},
	language = {en},
	number = {7766},
	urldate = {2025-08-05},
	journal = {Nature},
	author = {Arrangoiz-Arriola, Patricio and Wollack, E. Alex and Wang, Zhaoyou and Pechal, Marek and Jiang, Wentao and McKenna, Timothy P. and Witmer, Jeremy D. and Van Laer, Raphaël and Safavi-Naeini, Amir H.},
	month = jul,
	year = {2019},
	pages = {537--540},
	file = {Full Text PDF:C\:\\Users\\abarbero\\Zotero\\storage\\SSHZY9VE\\Arrangoiz-Arriola et al. - 2019 - Resolving the energy levels of a nanomechanical oscillator.pdf:application/pdf},
}

@article{tebbenjohanns_quantum_2021,
	title = {Quantum control of a nanoparticle optically levitated in cryogenic free space},
	volume = {595},
	copyright = {2021 The Author(s), under exclusive licence to Springer Nature Limited},
	issn = {1476-4687},
	url = {https://www.nature.com/articles/s41586-021-03617-w},
	doi = {10.1038/s41586-021-03617-w},
	abstract = {Tests of quantum mechanics on a macroscopic scale require extreme control over mechanical motion and its decoherence1–3. Quantum control of mechanical motion has been achieved by engineering the radiation–pressure coupling between a micromechanical oscillator and the electromagnetic field in a resonator4–7. Furthermore, measurement-based feedback control relying on cavity-enhanced detection schemes has been used to cool micromechanical oscillators to their quantum ground states8. In contrast to mechanically tethered systems, optically levitated nanoparticles are particularly promising candidates for matter-wave experiments with massive objects9,10, since their trapping potential is fully controllable. Here we optically levitate a femtogram (10−15 grams) dielectric particle in cryogenic free space, which suppresses thermal effects sufficiently to make the measurement backaction the dominant decoherence mechanism. With an efficient quantum measurement, we exert quantum control over the dynamics of the particle. We cool its centre-of-mass motion by measurement-based feedback to an average occupancy of 0.65 motional quanta, corresponding to a state purity of 0.43. The absence of an optical resonator and its bandwidth limitations holds promise to transfer the full quantum control available for electromagnetic fields to a mechanical system. Together with the fact that the optical trapping potential is highly controllable, our experimental platform offers a route to investigating quantum mechanics at macroscopic scales11.},
	language = {en},
	number = {7867},
	urldate = {2025-08-05},
	journal = {Nature},
	author = {Tebbenjohanns, Felix and Mattana, M. Luisa and Rossi, Massimiliano and Frimmer, Martin and Novotny, Lukas},
	month = jul,
	year = {2021},
	pages = {378--382},
	file = {Full Text PDF:C\:\\Users\\abarbero\\Zotero\\storage\\ZXPXZESL\\Tebbenjohanns et al. - 2021 - Quantum control of a nanoparticle optically levitated in cryogenic free space.pdf:application/pdf},
}

@article{mayor_high_2025,
	title = {High photon-phonon pair generation rate in a two-dimensional optomechanical crystal},
	volume = {16},
	copyright = {2025 The Author(s)},
	issn = {2041-1723},
	url = {https://www.nature.com/articles/s41467-025-57948-7},
	doi = {10.1038/s41467-025-57948-7},
	abstract = {Integrated optomechanical systems are a leading platform for manipulating, sensing, and distributing quantum information, but are limited by residual optical heating. Here, we demonstrate a two-dimensional optomechanical crystal (OMC) geometry with increased thermal anchoring and a mechanical mode at 7.4 GHz, well aligned with the operation range of cryogenic microwave hardware and piezoelectric transducers. The eight times better thermalization than current one-dimensional OMCs, large optomechanical coupling rates, g0/2π  ≈  880 kHz, and high optical quality factors, Qopt = 2.4 × 105, allow ground-state cooling (nm = 0.32) of the acoustic mode from 3 K and entering the optomechanical strong-coupling regime. In pulsed sideband asymmetry measurements, we show ground-state operation (nm {\textless} 0.45) at temperatures below 10 mK, with repetition rates up to 3 MHz, generating photon-phonon pairs at  ≈ 147 kHz. Our results extend optomechanical system capabilities and establish a robust foundation for future microwave-to-optical transducers with entanglement rates exceeding state-of-the-art superconducting qubit decoherence rates.},
	language = {en},
	number = {1},
	urldate = {2025-08-05},
	journal = {Nature Communications},
	author = {Mayor, Felix M. and Malik, Sultan and Primo, André G. and Gyger, Samuel and Jiang, Wentao and Alegre, Thiago P. M. and Safavi-Naeini, Amir H.},
	month = mar,
	year = {2025},
	pages = {2576},
	file = {Full Text PDF:C\:\\Users\\abarbero\\Zotero\\storage\\STCMDJMB\\Mayor et al. - 2025 - High photon-phonon pair generation rate in a two-dimensional optomechanical crystal.pdf:application/pdf},
}

@article{ding_high_2010,
	title = {High {Frequency} {GaAs} {Nano}-{Optomechanical} {Disk} {Resonator}},
	volume = {105},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.105.263903},
	doi = {10.1103/PhysRevLett.105.263903},
	abstract = {Optomechanical coupling between a mechanical oscillator and light trapped in a cavity increases when the coupling takes place in a reduced volume. Here we demonstrate a GaAs semiconductor optomechanical disk system where both optical and mechanical energy can be confined in a subwavelength scale interaction volume. We observe a giant optomechanical coupling rate up to 100 GHz/nm involving picogram mass mechanical modes with a frequency between 100 MHz and 1 GHz. The mechanical modes are singled-out measuring their dispersion as a function of disk geometry. Their Brownian motion is optically resolved with a sensitivity of 10−17 m/√Hz at room temperature and pressure, approaching the quantum limit imprecision.},
	number = {26},
	urldate = {2025-07-01},
	journal = {Physical Review Letters},
	author = {Ding, Lu and Baker, Christophe and Senellart, Pascale and Lemaitre, Aristide and Ducci, Sara and Leo, Giuseppe and Favero, Ivan},
	month = dec,
	year = {2010},
	pages = {263903},
	file = {APS Snapshot:C\:\\Users\\abarbero\\Zotero\\storage\\KNTBAUWE\\PhysRevLett.105.html:text/html;Version soumise:C\:\\Users\\abarbero\\Zotero\\storage\\GEBZMPD2\\Ding et al. - 2010 - High Frequency GaAs Nano-Optomechanical Disk Resonator.pdf:application/pdf},
}

@article{neshasteh_optomechanical_2025,
	title = {Optomechanical micro-rheology of complex fluids at ultra-high frequency},
	volume = {16},
	copyright = {2024 The Author(s)},
	issn = {2041-1723},
	url = {https://www.nature.com/articles/s41467-024-54522-5},
	doi = {10.1038/s41467-024-54522-5},
	abstract = {We present an optomechanical method for locally measuring the rheological properties of complex fluids in the ultra-high frequency range (UHF). A mechanical disk of microscale volume is used as an oscillating probe that monitors a liquid at rest, while the oscillation is optomechanically transduced. An analytical model for fluid-structure interactions is used to deduce the rheological properties of the liquid. This method is calibrated on liquid water, which despite pronounced compressibility effects remains Newtonian over the explored range. In contrast, liquid 1-decanol exhibits a non-Newtonian behavior, with a frequency-dependent viscosity showing two relaxation times of 797 and 151 picoseconds, associated to supramolecular and intramolecular processes. A shear elastic response appears at the highest frequencies, whose value allows determining the volume of a single liquid molecule. UHF optomechanical micro-rheology provides direct mechanical access to the fast molecular dynamics in a liquid, in a quantitative manner and within a sub-millisecond measurement time.},
	language = {en},
	number = {1},
	urldate = {2025-08-13},
	journal = {Nature Communications},
	author = {Neshasteh, H. and Shlesinger, I. and Ravaro, M. and Gély, M. and Jourdan, G. and Hentz, S. and Favero, I.},
	month = jan,
	year = {2025},
	pages = {407},
	file = {Full Text PDF:C\:\\Users\\abarbero\\Zotero\\storage\\HW6DJK93\\Neshasteh et al. - 2025 - Optomechanical micro-rheology of complex fluids at ultra-high frequency.pdf:application/pdf},
}

@article{de_oliveira_whispering-gallery_2024,
	title = {Whispering-{Gallery} {Quantum}-{Well} {Exciton} {Polaritons} in an {Indium} {Gallium} {Arsenide} {Microdisk} {Cavity}},
	volume = {132},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.132.126901},
	doi = {10.1103/PhysRevLett.132.126901},
	abstract = {Despite appealing high-symmetry properties that enable strong spatial confinement and ultrahigh-��, optical whispering-gallery modes of spherical and circular resonators have been absent from the field of quantum-well exciton polaritons. Here we observe whispering-gallery exciton polaritons in a gallium arsenide microdisk cavity filled with indium gallium arsenide quantum wells, the test bed materials of polaritonics. Strong coupling is evidenced in photoluminescence and resonant spectroscopy accessed through concomitant confocal microscopy and near-field optical techniques. Excitonic and optical resonances are tuned by varying temperature and disk radius, revealing Rabi splittings between 5 and 10 meV. A dedicated analytical quantum model for such circular whispering-gallery polaritons is developed, which reproduces the measured values. At high power, lasing is observed and accompanied by a blueshift of the emission consistent with the regime of polariton lasing. With experimental methods and theory now established, whispering-gallery-mode polaritons in round dielectric resonators appear as a new viable platform toward low loss polaritonics.},
	number = {12},
	urldate = {2025-08-13},
	journal = {Physical Review Letters},
	author = {de Oliveira, Romain and Colombano, Martin and Malabat, Florent and Morassi, Martina and Lemaître, Aristide and Favero, Ivan},
	month = mar,
	year = {2024},
	pages = {126901},
	file = {APS Snapshot:C\:\\Users\\abarbero\\Zotero\\storage\\NJET8UC3\\PhysRevLett.132.html:text/html;Full Text PDF:C\:\\Users\\abarbero\\Zotero\\storage\\XQN8B22R\\de Oliveira et al. - 2024 - Whispering-Gallery Quantum-Well Exciton Polaritons in an Indium Gallium Arsenide Microdisk Cavity.pdf:application/pdf},
}

@article{carlon_zambon_enhanced_2022,
	title = {Enhanced {Cavity} {Optomechanics} with {Quantum}-{Well} {Exciton} {Polaritons}},
	volume = {129},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.129.093603},
	doi = {10.1103/PhysRevLett.129.093603},
	abstract = {Semiconductor microresonators embedding quantum wells can host tightly confined and mutually interacting excitonic, optical, and mechanical modes at once. We theoretically investigate the case where the system operates in the strong exciton-photon coupling regime, while the optical and excitonic resonances are parametrically modulated by the interaction with a mechanical mode. Owing to the large exciton-phonon coupling at play in semiconductors, we predict an enhancement of polariton-phonon interactions by 2 orders of magnitude with respect to mere optomechanical coupling: a near-unity single-polariton quantum cooperativity is within reach for current semiconductor resonator platforms. We further analyze how polariton nonlinearities affect dynamical backaction, modifying the capability to cool or amplify the mechanical motion.},
	number = {9},
	urldate = {2025-08-13},
	journal = {Physical Review Letters},
	author = {Carlon Zambon, N. and Denis, Z. and De Oliveira, R. and Ravets, S. and Ciuti, C. and Favero, I. and Bloch, J.},
	month = aug,
	year = {2022},
	pages = {093603},
	file = {APS Snapshot:C\:\\Users\\abarbero\\Zotero\\storage\\GN5SASDL\\PhysRevLett.129.html:text/html;Full Text PDF:C\:\\Users\\abarbero\\Zotero\\storage\\UJX892GP\\Carlon Zambon et al. - 2022 - Enhanced Cavity Optomechanics with Quantum-Well Exciton Polaritons.pdf:application/pdf},
}

@article{sbarra_multimode_2022,
	title = {Multimode {Optomechanical} {Weighting} of a {Single} {Nanoparticle}},
	volume = {22},
	issn = {1530-6984},
	url = {https://doi.org/10.1021/acs.nanolett.1c03890},
	doi = {10.1021/acs.nanolett.1c03890},
	abstract = {We demonstrate multimode optomechanical sensing of individual nanoparticles with a radius between 75 and 150 nm. A semiconductor optomechanical disk resonator is optically driven and detected under ambient conditions, as nebulized nanoparticles land on it. Multiple mechanical and optical resonant signals of the disk are tracked simultaneously, providing access to several pieces of physical information about the landing analyte in real time. Thanks to a fast camera registering the time and position of landing, these signals can be employed to weight each nanoparticle with precision. Sources of error and deviation are discussed and modeled, indicating a path to evaluate the elasticity of the nanoparticles on top of their mere mass. The device is optimized for the future investigation of biological particles in the high megadalton range, such as large viruses.},
	number = {2},
	urldate = {2025-08-13},
	journal = {Nano Letters},
	author = {Sbarra, Samantha and Waquier, Louis and Suffit, Stephan and Lemaître, Aristide and Favero, Ivan},
	month = jan,
	year = {2022},
	pages = {710--715},
	file = {Version soumise:C\:\\Users\\abarbero\\Zotero\\storage\\3B5SPFHT\\Sbarra et al. - 2022 - Multimode Optomechanical Weighting of a Single Nanoparticle.pdf:application/pdf},
}

@article{guha_surface-enhanced_2017,
	title = {Surface-enhanced gallium arsenide photonic resonator with quality factor of 6 × 10$^{\textrm{6}}$},
	volume = {4},
	copyright = {© 2017 Optical Society of America},
	issn = {2334-2536},
	url = {https://opg.optica.org/optica/abstract.cfm?uri=optica-4-2-218},
	doi = {10.1364/OPTICA.4.000218},
	abstract = {Gallium arsenide and related compound semiconductors lie at the heart of optoelectronics and integrated laser technologies. Shaped at the micro- and nanoscale, they allow strong interaction with quantum dots and quantum wells, and promise stunning optically active devices. However, gallium arsenide optical structures presently exhibit lower performance than their passive counterparts based on silicon, notably in nanophotonics, where the surface plays a chief role. Here, we report on advanced surface control of miniature gallium arsenide optical resonators using two distinct techniques that produce permanent results. One extends the lifetime of free carriers and enhances luminescence, while the other strongly reduces surface absorption and enables ultra-low optical dissipation devices. With such surface control, the quality factor of wavelength-sized optical disk resonators is observed to rise up to 6\&\#x00D7;106 at the telecom wavelength, greatly surpassing previous realizations and opening new prospects for gallium arsenide nanophotonics.},
	language = {EN},
	number = {2},
	urldate = {2025-06-30},
	journal = {Optica},
	author = {Guha, Biswarup and Marsault, Felix and Cadiz, Fabian and Morgenroth, Laurence and Ulin, Vladimir and Berkovitz, Vladimir and Lemaître, Aristide and Gomez, Carmen and Amo, Alberto and Combrié, Sylvain and Gérard, Bruno and Leo, Giuseppe and Favero, Ivan},
	month = feb,
	year = {2017},
	pages = {218--221},
	file = {Version soumise:C\:\\Users\\abarbero\\Zotero\\storage\\ATFRXF7X\\Guha et al. - 2017 - Surface-enhanced gallium arsenide photonic resonator with quality factor of 6 × 106.pdf:application/pdf},
}

@article{najer_suppression_2021,
	title = {Suppression of {Surface}-{Related} {Loss} in a {Gated} {Semiconductor} {Microcavity}},
	volume = {15},
	url = {https://link.aps.org/doi/10.1103/PhysRevApplied.15.044004},
	doi = {10.1103/PhysRevApplied.15.044004},
	abstract = {We present a surface-passivation method that reduces surface-related losses by almost 2 orders of magnitude in a highly miniaturized Ga⁢As open microcavity. The microcavity consists of a curved dielectric distributed Bragg reflector with radius of approximately 10 ��⁢m paired with a Ga⁢As-based heterostructure. The heterostructure consists of a semiconductor distributed Bragg reflector followed by an ��-��-�� diode with a layer of quantum dots in the intrinsic region. Free-carrier absorption in the highly-��-doped and highly-��-doped layers is minimized by our positioning them close to a node of the vacuum electromagnetic field. The surface, however, resides at an antinode of the vacuum field and results in significant loss. These losses are much reduced by surface passivation. The strong dependence on wavelength implies that the main effect of the surface passivation is to eliminate the surface electric field, thereby quenching below-band-gap absorption via a Franz-Keldysh-like effect. An additional benefit is that the surface passivation reduces scattering at the Ga⁢As surface. These results are important in other nanophotonic devices that rely on a Ga⁢As-vacuum interface to confine the electromagnetic field.},
	number = {4},
	urldate = {2025-06-30},
	journal = {Physical Review Applied},
	author = {Najer, Daniel and Tomm, Natasha and Javadi, Alisa and Korsch, Alexander R. and Petrak, Benjamin and Riedel, Daniel and Dolique, Vincent and Valentin, Sascha R. and Schott, Rüdiger and Wieck, Andreas D. and Ludwig, Arne and Warburton, Richard J.},
	month = apr,
	year = {2021},
	pages = {044004},
	file = {APS Snapshot:C\:\\Users\\abarbero\\Zotero\\storage\\PWFHC2VE\\PhysRevApplied.15.html:text/html;Texte intégral:C\:\\Users\\abarbero\\Zotero\\storage\\6TK9RTDZ\\Najer et al. - 2021 - Suppression of Surface-Related Loss in a Gated Semiconductor Microcavity.pdf:application/pdf},
}

@article{pautrel_efficient_2024,
	title = {Efficient and stable coupling to nanophotonic waveguides and resonators in stringent environments},
	volume = {32},
	copyright = {© 2024 Optica Publishing Group},
	issn = {1094-4087},
	url = {https://opg.optica.org/oe/abstract.cfm?uri=oe-32-15-26954},
	doi = {10.1364/OE.521697},
	abstract = {Using conical optical fibers, we explore new methods for coupling light to nanophotonic structures operated in constrained environments. With a single-sided conical fiber taper, we demonstrate efficient coupling to an on-chip nanophotonic bus waveguide immersed in a liquid. In the aim of coupling light into a target whispering gallery disk resonator, we then replace such on-chip nanophotonic bus waveguide with two conical fibers joined face to face. This latter approach leads to highly efficient coupling superior to 90\&\#x0025; and is shown to be stable within a vibrating pulse tube cryostat operating at low temperatures. It is demonstrated in the telecom band and in the near infrared close to 900 nm of wavelength. Conical fiber methods hence enable reaching the coupling performances required in quantum optics or sensing experiments, even in stringent environments where signal-to-noise had remained a challenge.},
	language = {EN},
	number = {15},
	urldate = {2025-05-13},
	journal = {Optics Express},
	author = {Pautrel, S. and Malabat, F. and Waquier, L. and Colombano, M. and Morassi, M. and Lemaître, A. and Favero, I.},
	month = jul,
	year = {2024},
	pages = {26954--26963},
	file = {Full Text PDF:C\:\\Users\\abarbero\\Zotero\\storage\\RDQFS5MF\\Pautrel et al. - 2024 - Efficient and stable coupling to nanophotonic waveguides and resonators in stringent environments.pdf:application/pdf},
}

@article{borselli_beyond_2005,
	title = {Beyond the {Rayleigh} scattering limit in high-{Q} silicon microdisks: theory and experiment},
	volume = {13},
	copyright = {© 2005 Optical Society of America},
	issn = {1094-4087},
	shorttitle = {Beyond the {Rayleigh} scattering limit in high-{Q} silicon microdisks},
	url = {https://opg.optica.org/oe/abstract.cfm?uri=oe-13-5-1515},
	doi = {10.1364/OPEX.13.001515},
	abstract = {Using a combination of resist reflow to form a highly circular etch mask pattern and a low-damage plasma dry etch, high-quality-factor silicon optical microdisk resonators are fabricated out of silicon-oninsulator (SOI) wafers. Quality factors as high as Q=5×106 are measured in these microresonators, corresponding to a propagation loss coefficient as small as α{\textasciitilde}0.1 dB/cm. The different optical loss mechanisms are identified through a study of the total optical loss, mode coupling, and thermally-induced optical bistability as a function of microdisk radius (5-30 µm). These measurements indicate that optical loss in these high-Q microresonators is limited not by surface roughness, but rather by surface state absorption and bulk free-carrier absorption.},
	language = {EN},
	number = {5},
	urldate = {2025-04-04},
	journal = {Optics Express},
	author = {Borselli, Matthew and Johnson, Thomas J. and Painter, Oskar},
	month = mar,
	year = {2005},
	pages = {1515--1530},
	file = {Full Text PDF:C\:\\Users\\abarbero\\Zotero\\storage\\HQH2NJ26\\Borselli et al. - 2005 - Beyond the Rayleigh scattering limit in high-Q silicon microdisks theory and experiment.pdf:application/pdf},
}

@article{guha_force_2020,
	title = {Force {Sensing} with an {Optomechanical} {Self}-{Oscillator}},
	volume = {14},
	url = {https://link.aps.org/doi/10.1103/PhysRevApplied.14.024079},
	doi = {10.1103/PhysRevApplied.14.024079},
	abstract = {Ultra-high-frequency nanomechanical resonators (���� {\textgreater}300 MHz) can increase our capacity to study fast physical phenomena, for example by measuring forces. Their extreme stiffness is also a chance to access molecular forces in the subpicometer low amplitude of motion limit, but it makes them hard to drive and control. Here we analyze a method to optomechanically sense a force field with an ultra-high-frequency and stiff mechanical resonator, where back-action optical forces set the resonator into a self-sustained stable oscillator trajectory. After elucidating the experimental conditions to obtain optimal resolution, we carry out controlled experiments where the oscillator senses an optical force generated by a secondary laser. We analyze and model our results, and illustrate the concrete advantage of the method in the measurement of such a weak force, which would otherwise remain undetected by the undriven probe. We establish the thermodynamical limits of the approach, and finally connect it to the class of feedback-controlled problems, clarifying its assets and limitations.},
	number = {2},
	urldate = {2025-10-01},
	journal = {Physical Review Applied},
	author = {Guha, Biswarup and Allain, Pierre Etienne and Lemaître, Aristide and Leo, Giuseppe and Favero, Ivan},
	month = aug,
	year = {2020},
	pages = {024079},
	file = {APS Snapshot:C\:\\Users\\abarbero\\Zotero\\storage\\WNK4TQD3\\PhysRevApplied.14.html:text/html;Full Text PDF:C\:\\Users\\abarbero\\Zotero\\storage\\DPRHF554\\Guha et al. - 2020 - Force Sensing with an Optomechanical Self-Oscillator.pdf:application/pdf},
}

@article{allain_optomechanical_2020,
	title = {Optomechanical resonating probe for very high frequency sensing of atomic forces},
	volume = {12},
	issn = {2040-3372},
	url = {https://pubs.rsc.org/en/content/articlelanding/2020/nr/c9nr09690f},
	doi = {10.1039/C9NR09690F},
	abstract = {Atomic force spectroscopy and microscopy are invaluable tools to characterize nanostructures and biological systems. State-of-the-art experiments use resonant driving of mechanical probes, whose frequency reaches MHz in the fastest commercial instruments where cantilevers are driven at nanometer amplitude. Stiffer probes oscillating at tens of picometers provide a better access to short-range interactions, yielding images of molecular bonds, but they are little amenable to high-speed operation. Next-generation investigations demand combining very high frequency ({\textgreater}100 MHz) with deep sub-nanometer oscillation amplitude, in order to access faster (below microsecond) phenomena with molecular resolution. Here we introduce a resonating optomechanical atomic force probe operated fully optically at a frequency of 117 MHz, two decades above cantilevers, with a Brownian motion amplitude four orders below. Based on Silicon-On-Insulator technology, the very high frequency probe demonstrates single-pixel sensing of contact and non-contact interactions with sub-picometer amplitude, breaking open current limitations for faster and finer force spectroscopy.},
	language = {en},
	number = {5},
	urldate = {2025-10-01},
	journal = {Nanoscale},
	author = {Allain, Pierre Etienne and Schwab, Lucien and Mismer, Colin and Gely, Marc and Mairiaux, Estelle and Hermouet, Maxime and Walter, Benjamin and Leo, Giuseppe and Hentz, Sébastien and Faucher, Marc and Jourdan, Guillaume and Legrand, Bernard and Favero, Ivan},
	month = feb,
	year = {2020},
	pages = {2939--2945},
	file = {Supplementary Information PDF:C\:\\Users\\abarbero\\Zotero\\storage\\W6AYKILE\\Allain et al. - 2020 - Optomechanical resonating probe for very high frequency sensing of atomic forces.pdf:application/pdf},
}

@article{meenehan_pulsed_2015,
	title = {Pulsed {Excitation} {Dynamics} of an {Optomechanical} {Crystal} {Resonator} near {Its} {Quantum} {Ground} {State} of {Motion}},
	volume = {5},
	url = {https://link.aps.org/doi/10.1103/PhysRevX.5.041002},
	doi = {10.1103/PhysRevX.5.041002},
	abstract = {Using pulsed optical excitation and read-out along with single-phonon-counting techniques, we measure the transient backaction, heating, and damping dynamics of a nanoscale silicon optomechanical crystal cavity mounted in a dilution refrigerator at a base temperature of ����≈11 mK. In addition to observing a slow (approximately 740-ns) turn-on time for the optical-absorption-induced hot-phonon bath, we measure for the 5.6-GHz “breathing” acoustic mode of the cavity an initial phonon occupancy as low as ⟨��⟩ =0.021 ±0.007 (mode temperature ��min ≈70 mK) and an intrinsic mechanical decay rate of ��0 = 328 ±14 Hz (���� ≈1.7 ×107). These measurements demonstrate the feasibility of using short pulsed measurements for a variety of quantum optomechanical applications despite the presence of steady-state optical heating.},
	number = {4},
	urldate = {2025-04-10},
	journal = {Physical Review X},
	author = {Meenehan, Seán M. and Cohen, Justin D. and MacCabe, Gregory S. and Marsili, Francesco and Shaw, Matthew D. and Painter, Oskar},
	month = oct,
	year = {2015},
	pages = {041002},
	file = {APS Snapshot:C\:\\Users\\abarbero\\Zotero\\storage\\QU5N2LF7\\PhysRevX.5.html:text/html;Full Text PDF:C\:\\Users\\abarbero\\Zotero\\storage\\96JEN5GF\\Meenehan et al. - 2015 - Pulsed Excitation Dynamics of an Optomechanical Crystal Resonator near Its Quantum Ground State of M.pdf:application/pdf},
}

@article{cohen_phonon_2015,
	title = {Phonon counting and intensity interferometry of a nanomechanical resonator},
	volume = {520},
	copyright = {2015 Springer Nature Limited},
	issn = {1476-4687},
	url = {https://www.nature.com/articles/nature14349},
	doi = {10.1038/nature14349},
	abstract = {A silicon nanometre-scale mechanical resonator, patterned to couple optical and mechanical resonances, is found to emit photons when optically pumped; photon emission corresponds directly to phonon emission, enabling the phonons to be counted.},
	language = {en},
	number = {7548},
	urldate = {2025-04-10},
	journal = {Nature},
	author = {Cohen, Justin D. and Meenehan, Seán M. and MacCabe, Gregory S. and Gröblacher, Simon and Safavi-Naeini, Amir H. and Marsili, Francesco and Shaw, Matthew D. and Painter, Oskar},
	month = apr,
	year = {2015},
	pages = {522--525},
	file = {Full Text PDF:C\:\\Users\\abarbero\\Zotero\\storage\\86Y934AU\\Cohen et al. - 2015 - Phonon counting and intensity interferometry of a nanomechanical resonator.pdf:application/pdf},
}

@article{poot_mechanical_2012,
	series = {Mechanical systems in the quantum regime},
	title = {Mechanical systems in the quantum regime},
	volume = {511},
	issn = {0370-1573},
	url = {https://www.sciencedirect.com/science/article/pii/S0370157311003644},
	doi = {10.1016/j.physrep.2011.12.004},
	abstract = {Mechanical systems are ideal candidates for studying quantum behavior of macroscopic objects. To this end, a mechanical resonator has to be cooled to its ground state and its position has to be measured with great accuracy. Currently, various routes to reach these goals are being explored. In this review, we discuss different techniques for sensitive position detection and we give an overview of the cooling techniques that are being employed. The latter includes sideband cooling and active feedback cooling. The basic concepts that are important when measuring on mechanical systems with high accuracy and/or at very low temperatures, such as thermal and quantum noise, linear response theory, and backaction, are explained. From this, the quantum limit on linear position detection is obtained and the sensitivities that have been achieved in recent opto- and nanoelectromechanical experiments are compared to this limit. The mechanical resonators that are used in the experiments range from meter-sized gravitational wave detectors to nanomechanical systems that can only be read out using mesoscopic devices such as single-electron transistors or superconducting quantum interference devices. A special class of nanomechanical systems is bottom-up fabricated carbon-based devices, which have very high frequencies and yet a large zero-point motion, making them ideal for reaching the quantum regime. The mechanics of some of the different mechanical systems at the nanoscale is studied. We conclude this review with an outlook of how state-of-the-art mechanical resonators can be improved to study quantum mechanics.},
	number = {5},
	urldate = {2025-08-13},
	journal = {Physics Reports},
	author = {Poot, Menno and van der Zant, Herre S. J.},
	month = feb,
	year = {2012},
	pages = {273--335},
}


@article{callaway_low-temperature_1961,
	title = {Low-{Temperature} {Lattice} {Thermal} {Conductivity}},
	volume = {122},
	url = {https://link.aps.org/doi/10.1103/PhysRev.122.787},
	doi = {10.1103/PhysRev.122.787},
	abstract = {The effect of point imperfections on lattice thermal conductivity is discussed with particular attention to the case in which the temperature is low but the normal three-phonon scattering is still dominant. The experimental results of Walker and Fairbank on the conductivity of isotopic mixtures of solid helium are analyzed.},
	number = {3},
	urldate = {2025-08-14},
	journal = {Physical Review},
	author = {Callaway, Joseph},
	month = may,
	year = {1961},
	pages = {787--790},
	file = {APS Snapshot:C\:\\Users\\abarbero\\Zotero\\storage\\LMA3GG9D\\PhysRev.122.html:text/html;Full Text PDF:C\:\\Users\\abarbero\\Zotero\\storage\\DKHVUGL4\\Callaway - 1961 - Low-Temperature Lattice Thermal Conductivity.pdf:application/pdf},
}

@article{agrawal_lattice_1962,
	title = {Lattice {Thermal} {Conductivity} at {Low} {Temperatures}},
	volume = {126},
	url = {https://link.aps.org/doi/10.1103/PhysRev.126.24},
	doi = {10.1103/PhysRev.126.24},
	abstract = {The theoretical models of Callaway and Klemens are compared to experimental results in (a) silicon and diamond, (b) solidified argon and neon, and (c) KCl and NaF, which are taken from the literature. Three sources of scattering are postulated: phonon-phonon processes, isotopic point defect scattering, and boundary scattering, except in NaF where isotopic scattering is absent. The Callaway model, in all cases, gives a good fit and excellent agreement is obtained for diamond and solidified argon and neon. In the vicinity of the conductivity maxima the Callaway model gives a better fit with the experimental curve. The disagreement between the results of the two models is most pronounced in solidified argon and neon where the Debye temperature is low and Umklapp processes are predominant at the conductivity maximum. In diamond, where the Debye temperature is quite high and Umklapp processes are unimportant at the temperatures of interest the results of both models are more or less similar. The Casimir model for finding the characteristic length for the boundary scattering fails to explain the observed results in solidified argon and neon. This indicates the existence of microscale fluctuations in the composition of the solid. In NaF the characteristic length has to be decreased by a factor of about 5. For diamond the value of the parameter ��, which gives the best fit with experiment, is a hundred times the value calculated from Klemens' expression for ��. This supports the earlier suggestion that there occur clusters of point defects in diamond. Good agreement with the experimental results beyond the conductivity maximum is obtained by taking (��1 +��2) to be temperature independent in all the cases.},
	number = {1},
	urldate = {2025-08-14},
	journal = {Physical Review},
	author = {Agrawal, Bal Krishna and Verma, G. S.},
	month = apr,
	year = {1962},
	pages = {24--29},
	file = {APS Snapshot:C\:\\Users\\abarbero\\Zotero\\storage\\QAMWAZEU\\PhysRev.126.html:text/html;Full Text PDF:C\:\\Users\\abarbero\\Zotero\\storage\\B5C7K8Q4\\Agrawal et Verma - 1962 - Lattice Thermal Conductivity at Low Temperatures.pdf:application/pdf},
}

@article{klemens_thermal_1997,
	title = {The thermal conductivity of dielectric solids at low temperatures ({Theoretical})},
	volume = {208},
	url = {https://royalsocietypublishing.org/doi/10.1098/rspa.1951.0147},
	doi = {10.1098/rspa.1951.0147},
	abstract = {The statistical equilibrium of phonons in the presence of a temperature gradient is investigated, and a general formula for the thermal conductivity of dielectric solids is obtained. This is applied to quartz glass, giving good agreement with values observed by Berman (1951), and to crystals. Comparison between theory and experiment are made for alkali-halides and quartz, and conclusions are drawn about the defects in neutron-irradiated quartz.},
	number = {1092},
	urldate = {2025-08-14},
	journal = {Proceedings of the Royal Society of London. Series A. Mathematical and Physical Sciences},
	author = {Klemens, P. G.},
	month = jan,
	year = {1997},
	pages = {108--133},
	file = {Full Text PDF:C\:\\Users\\abarbero\\Zotero\\storage\\YBL28WIM\\Klemens - 1997 - The thermal conductivity of dielectric solids at low temperatures (Theoretical).pdf:application/pdf},
}

@article{sun_high-q_2012,
	title = {High-{Q} silicon optomechanical microdisk resonators at gigahertz frequencies},
	volume = {100},
	issn = {0003-6951},
	url = {https://doi.org/10.1063/1.4709416},
	doi = {10.1063/1.4709416},
	abstract = {We report disk-shaped silicon optomechanical resonators with frequency up to 1.75 GHz in the ultrahigh frequency band. Optical transduction of the thermal motion of the disks’ in-plane vibrational modes yields a displacement sensitivity of 4.1 × 10−17 m/Hz1/2. Due to the reduced clamping loss, these disk resonators possess high mechanical quality factors (Q), with the highest value of 4370 for the 1.47 GHz mode measured in ambient air. Numerical simulation on the modal frequency and mechanical Q for disks of varying undercut shows modal coupling and suggests a realistic pedestal size to achieve the highest possible Q.},
	number = {17},
	urldate = {2025-09-03},
	journal = {Applied Physics Letters},
	author = {Sun, Xiankai and Zhang, Xufeng and Tang, Hong X.},
	month = apr,
	year = {2012},
	pages = {173116},
	file = {Snapshot:C\:\\Users\\abarbero\\Zotero\\storage\\8F2HGYJH\\1.html:text/html},
}

@article{gil-santos_optomechanical_2020,
	title = {Optomechanical detection of vibration modes of a single bacterium},
	volume = {15},
	copyright = {2020 The Author(s), under exclusive licence to Springer Nature Limited},
	issn = {1748-3395},
	url = {https://www.nature.com/articles/s41565-020-0672-y},
	doi = {10.1038/s41565-020-0672-y},
	abstract = {Low-frequency vibration modes of biological particles, such as proteins, viruses and bacteria, involve coherent collective vibrations at frequencies in the terahertz and gigahertz domains. These vibration modes carry information on their structure and mechanical properties, which are good indicators of their biological state. In this work, we harnessed a particular regime in the physics of coupled mechanical resonators to directly measure these low-frequency mechanical resonances of a single bacterium. We deposit the bacterium on the surface of an ultrahigh frequency optomechanical disk resonator in ambient conditions. The vibration modes of the disk and bacterium hybridize when their associated frequencies are similar. We developed a general theoretical framework to describe this coupling, which allows us to retrieve the eigenfrequencies and mechanical loss of the bacterium low-frequency vibration modes (quality factor). Additionally, we analysed the effect of hydration on these vibrational modes. This work demonstrates that ultrahigh frequency optomechanical resonators can be used for vibrational spectrometry with the unique capability to obtain information on single biological entities.},
	language = {en},
	number = {6},
	urldate = {2025-09-03},
	journal = {Nature Nanotechnology},
	author = {Gil-Santos, Eduardo and Ruz, Jose J. and Malvar, Oscar and Favero, Ivan and Lemaître, Aristide and Kosaka, Priscila M. and García-López, Sergio and Calleja, Montserrat and Tamayo, Javier},
	month = jun,
	year = {2020},
	pages = {469--474},
	file = {Full Text PDF:C\:\\Users\\abarbero\\Zotero\\storage\\R329VKWK\\Gil-Santos et al. - 2020 - Optomechanical detection of vibration modes of a single bacterium.pdf:application/pdf},
}

@article{lamberti_real-time_2022,
	title = {Real-{Time} {Sensing} with {Multiplexed} {Optomechanical} {Resonators}},
	volume = {22},
	issn = {1530-6984},
	url = {https://doi.org/10.1021/acs.nanolett.1c04017},
	doi = {10.1021/acs.nanolett.1c04017},
	abstract = {Nanoelectromechanical resonators have been successfully used for a variety of sensing applications. Their extreme resolution comes from their small size, which strongly limits their capture area. This leads to a long analysis time and the requirement for large sample quantity. Moreover, the efficiency of the electrical transductions commonly used for silicon resonators degrades with increasing frequency, limiting the achievable mechanical bandwidth and throughput. Multiplexing a large number of high-frequency resonators appears to be a solution, but this is complex with electrical transductions. We propose here a route to solve these issues, with a multiplexing scheme for very high-frequency optomechanical resonators. We demonstrate the simultaneous frequency measurement of three silicon microdisks fabricated with a 200 mm wafer large-scale process. The readout architecture is simple and does not degrade the sensing resolutions. This paves the way toward the realization of sensors for multiparametric analysis with an extremely low limit of detection and response time.},
	number = {5},
	urldate = {2025-09-03},
	journal = {Nano Letters},
	author = {Lamberti, Fabrice-Roland and Palanchoke, Ujwol and Geurts, Thijs Peter Joseph and Gely, Marc and Regord, Sébastien and Banniard, Louise and Sansa, Marc and Favero, Ivan and Jourdan, Guillaume and Hentz, Sébastien},
	month = mar,
	year = {2022},
	pages = {1866--1873},
	file = {Version soumise:C\:\\Users\\abarbero\\Zotero\\storage\\MNP7RGR9\\Lamberti et al. - 2022 - Real-Time Sensing with Multiplexed Optomechanical Resonators.pdf:application/pdf},
}


@article{teufel_sideband_2011,
	title = {Sideband cooling of micromechanical motion to the quantum ground state},
	volume = {475},
	copyright = {2011 Springer Nature Limited},
	issn = {1476-4687},
	url = {https://www.nature.com/articles/nature10261},
	doi = {10.1038/nature10261},
	abstract = {It has been a long-standing goal in the field of cavity optomechanics to cool down a mechanical resonator to its motional quantum ground state by using light. Teufel et al. have now achieved just that with a recently developed system in which a drum-like flexible aluminium membrane is incorporated in a superconducting circuit. Ground-state cooling of a mechanical resonator was demonstrated for the first time last year in a different type of device, but the quantum states in this new device should be much longer lived, allowing direct tests of fundamental principles of quantum mechanics. As a first step, the authors perform a quantum-limited position measurement that is only a factor of about five away from the Heisenberg limit.},
	language = {en},
	number = {7356},
	urldate = {2025-08-27},
	journal = {Nature},
	author = {Teufel, J. D. and Donner, T. and Li, Dale and Harlow, J. W. and Allman, M. S. and Cicak, K. and Sirois, A. J. and Whittaker, J. D. and Lehnert, K. W. and Simmonds, R. W.},
	month = jul,
	year = {2011},
	pages = {359--363},
	file = {Full Text PDF:C\:\\Users\\abarbero\\Zotero\\storage\\WL9QQ9ET\\Teufel et al. - 2011 - Sideband cooling of micromechanical motion to the quantum ground state.pdf:application/pdf},
}

@article{peterson_laser_2016,
	title = {Laser {Cooling} of a {Micromechanical} {Membrane} to the {Quantum} {Backaction} {Limit}},
	volume = {116},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.116.063601},
	doi = {10.1103/PhysRevLett.116.063601},
	abstract = {The radiation pressure of light can act to damp and cool the vibrational motion of a mechanical resonator, but even if the light field has no thermal component, shot noise still sets a limit on the minimum phonon occupation. In optomechanical sideband cooling in a cavity, the finite off-resonant Stokes scattering defined by the cavity linewidth combined with shot noise fluctuations dictates a quantum backaction limit, analogous to the Doppler limit of atomic laser cooling. In our work, we sideband cool a micromechanical membrane resonator to the quantum backaction limit. Monitoring the optical sidebands allows us to directly observe the mechanical object come to thermal equilibrium with the optical bath. This level of optomechanical coupling that overwhelms the intrinsic thermal decoherence was not reached in previous ground-state cooling demonstrations.},
	number = {6},
	urldate = {2025-08-27},
	journal = {Physical Review Letters},
	author = {Peterson, R. W. and Purdy, T. P. and Kampel, N. S. and Andrews, R. W. and Yu, P.-L. and Lehnert, K. W. and Regal, C. A.},
	month = feb,
	year = {2016},
	pages = {063601},
	file = {APS Snapshot:C\:\\Users\\abarbero\\Zotero\\storage\\V3PIA8RJ\\PhysRevLett.116.html:text/html;Full Text PDF:C\:\\Users\\abarbero\\Zotero\\storage\\HDFPKE6M\\Peterson et al. - 2016 - Laser Cooling of a Micromechanical Membrane to the Quantum Backaction Limit.pdf:application/pdf},
}

@article{noguchi_ground_2016,
	title = {Ground state cooling of a quantum electromechanical system with a silicon nitride membrane in a {3D} loop-gap cavity},
	volume = {18},
	issn = {1367-2630},
	url = {https://dx.doi.org/10.1088/1367-2630/18/10/103036},
	doi = {10.1088/1367-2630/18/10/103036},
	abstract = {Cavity electro-(opto-)mechanics gives us a quantum tool to access mechanical modes in a massive object. Here we develop a quantum electromechanical system in which a vibrational mode of a SiNx membrane are coupled to a three-dimensional loop-gap superconducting microwave cavity. The tight confinement of the electric field across a mechanically compliant narrow-gap capacitor realizes the quantum strong coupling regime under a red-sideband pump field and the quantum ground state cooling of the mechanical mode. We also demonstrate strong coupling between two mechanical modes, which is induced by two-tone parametric drives and mediated by a virtual photon in the cavity.},
	language = {en},
	number = {10},
	urldate = {2025-08-05},
	journal = {New Journal of Physics},
	author = {Noguchi, Atsushi and Yamazaki, Rekishu and Ataka, Manabu and Fujita, Hiroyuki and Tabuchi, Yutaka and Ishikawa, Toyofumi and Usami, Koji and Nakamura, Yasunobu},
	month = oct,
	year = {2016},
	pages = {103036},
	file = {IOP Full Text PDF:C\:\\Users\\abarbero\\Zotero\\storage\\I22E2EUN\\Noguchi et al. - 2016 - Ground state cooling of a quantum electromechanical system with a silicon nitride membrane in a 3D l.pdf:application/pdf},
}

@article{oconnell_quantum_2010,
	title = {Quantum ground state and single-phonon control of a mechanical resonator},
	volume = {464},
	copyright = {2010 Macmillan Publishers Limited. All rights reserved},
	issn = {1476-4687},
	url = {https://www.nature.com/articles/nature08967},
	doi = {10.1038/nature08967},
	abstract = {Quantum mechanics provides a highly accurate description of a wide variety of physical systems. However, a demonstration that quantum mechanics applies equally to macroscopic mechanical systems has been a long-standing challenge, hindered by the difficulty of cooling a mechanical mode to its quantum ground state. The temperatures required are typically far below those attainable with standard cryogenic methods, so significant effort has been devoted to developing alternative cooling techniques. Once in the ground state, quantum-limited measurements must then be demonstrated. Here, using conventional cryogenic refrigeration, we show that we can cool a mechanical mode to its quantum ground state by using a microwave-frequency mechanical oscillator—a ‘quantum drum’—coupled to a quantum bit, which is used to measure the quantum state of the resonator. We further show that we can controllably create single quantum excitations (phonons) in the resonator, thus taking the first steps to complete quantum control of a mechanical system.},
	language = {en},
	number = {7289},
	urldate = {2025-08-27},
	journal = {Nature},
	author = {O’Connell, A. D. and Hofheinz, M. and Ansmann, M. and Bialczak, Radoslaw C. and Lenander, M. and Lucero, Erik and Neeley, M. and Sank, D. and Wang, H. and Weides, M. and Wenner, J. and Martinis, John M. and Cleland, A. N.},
	month = apr,
	year = {2010},
	pages = {697--703},
	file = {Full Text PDF:C\:\\Users\\abarbero\\Zotero\\storage\\NUUA7TAY\\O’Connell et al. - 2010 - Quantum ground state and single-phonon control of a mechanical resonator.pdf:application/pdf},
}

@article{wallucks_quantum_2020,
	title = {A quantum memory at telecom wavelengths},
	volume = {16},
	copyright = {2020 The Author(s), under exclusive licence to Springer Nature Limited},
	issn = {1745-2481},
	url = {https://www.nature.com/articles/s41567-020-0891-z},
	doi = {10.1038/s41567-020-0891-z},
	abstract = {Nanofabricated mechanical resonators are gaining significant momentum among potential quantum technologies due to their unique design freedom and independence from naturally occurring resonances. As their functionality is widely detached from material choice, they constitute ideal tools for transducers—intermediaries between different quantum systems—and as memory elements in conjunction with quantum communication and computing devices. Their capability to host ultra-long-lived phonon modes is particularity attractive for non-classical information storage, both for future quantum technologies and for fundamental tests of physics. Here, we demonstrate a Duan–Lukin–Cirac–Zoller-type mechanical quantum memory with an energy decay time of T1 ≈ 2 ms, which is controlled through an optical interface engineered to natively operate at telecom wavelengths. We further investigate the coherence of the memory, equivalent to the dephasing \$\$\{T\}\_\{2\}{\textasciicircum}\{* \}\$\$ for qubits, which has a power-dependent value between 15 and 112 μs. This demonstration is enabled by an optical scheme to create a superposition state of \$\${\textbackslash}left{\textbar}0{\textbackslash}right{\textbackslash}rangle +{\textbackslash}left{\textbar}1{\textbackslash}right{\textbackslash}rangle\$\$ mechanical excitations, with an arbitrary ratio between the vacuum and single-phonon components.},
	language = {en},
	number = {7},
	urldate = {2025-09-17},
	journal = {Nature Physics},
	author = {Wallucks, Andreas and Marinković, Igor and Hensen, Bas and Stockill, Robert and Gröblacher, Simon},
	month = jul,
	year = {2020},
	pages = {772--777},
	file = {Full Text PDF:C\:\\Users\\abarbero\\Zotero\\storage\\X6FWBDHF\\Wallucks et al. - 2020 - A quantum memory at telecom wavelengths.pdf:application/pdf},
}

